Focus for Free in Density-Based Counting

This work considers supervised learning to count from images and their corresponding point annotations. Where density-based counting methods typically use the point annotations only to create Gaussian-density maps, which act as the supervision signal, the starting point of this work is that point annotations have counting potential beyond density map generation. We introduce two methods that repurpose the available point annotations to enhance counting performance. The first is a counting-specific augmentation that leverages point annotations to simulate occluded objects in both input and density images to enhance the network's robustness to occlusions. The second method, foreground distillation, generates foreground masks from the point annotations, from which we train an auxiliary network on images with blacked-out backgrounds. By doing so, it learns to extract foreground counting knowledge without interference from the background. These methods can be seamlessly integrated with existing counting advances and are adaptable to different loss functions. We demonstrate complementary effects of the approaches, allowing us to achieve robust counting results even in challenging scenarios such as background clutter, occlusion, and varying crowd densities. Our proposed approach achieves strong counting results on multiple datasets, including ShanghaiTech Part\_A and Part\_B, UCF\_QNRF, JHU-Crowd++, and NWPU-Crowd.

==> temp.tex <==
\subsection{Multi-stage optimization}
\label{sec:loss}
The optimization of our counting framework consists of three parts. The first part is to train a binary segmentation network as introduced in Section \ref{sec:segmentation}. We introduce a per-pixel weighted focal loss~\cite{lin2017focal}:
\begin{equation}
 \begin{split}
\mathcal{L}_d(X) = \parallel f_r(X)-\tilde D \parallel_{1},
\end{split}
\label{eq:loss-mainbranch}
\end{equation}
where $\tilde D$ denotes the distilled density map as introduced in Section \ref{sec:density}. For binary segmentation, we propose a per-pixel weighted focal loss~\cite{lin2017focal} to obtain a supervised focus from segmentation for input image $X$:
\begin{equation}
\begin{split}
\mathcal{L}_s(X) = 
 \sum_{{l} \in \{0,1\}} -\alpha{^l} S^l (1-f_{s}(X))^{\gamma_s} log(f_{s}(X)),
\label{eq:focus-seg}
\end{split}
\end{equation}
where $\alpha{^l}=1-\frac{|S^l|}{|S|}$. The focal parameter $\gamma_s$ is set to 2 throughout this network, as recommended by~\cite{lin2017focal}.

The second part is to train an auxiliary network for density distillation, as introduced in Section \ref{sec:density}. For the density estimation, we use the $\ell_1$ loss:
\begin{equation}
 \begin{split}
\mathcal{L}_d(X) = \parallel f_r(X)-\tilde D \parallel_{1},
\end{split}
\label{eq:loss-mainbranch}
\end{equation}
where $\tilde D$ denotes the distilled density map as introduced in Section \ref{sec:density}.

The third part is to train our final counting network to estimate the density map. The loss function is defined as:
\begin{equation}
 \begin{split}
\mathcal{L}(X) =
\lambda_r \mathcal{L}_d(X)+ \lambda_c \mathcal{L}_c(X),
\label{eq:final-loss}
\end{split}
\end{equation}
where $\mathcal{L}_c(X)$ is loss for global density classification:
\begin{equation}
 \begin{split}
\mathcal{L}_c(X) = 
\sum_{{l} \in \{0,1,..,M\}} -G^l (1-f_{c}(X))^{\gamma_c} log(f_{c}(X)),
\label{eq:focus-compactness}
\end{split}
\end{equation}
where $\gamma_c$ is set to 2 as well.


\section{Focus for free}
\label{sec:method}

\cs{There is too much `focus-talk' in this section, if you call everything focus you may as well leave the word out. The information value becomes zero and irritates the reader.}

This work considers learning to count in a supervised manner, in which the training samples are provided as images and their corresponding point annotations. For density-based counting, the point annotations are generally used to generate Gaussian-density maps, which then serve as the supervision signal. This work starts from the premise that point annotations are a rich source of annotations with value for counting beyond generating density maps. We provide three ways to re-purpose the already available point annotations to improve the transformation from images to density maps in counting. Below, we start by introducing how to create a non-uniform Gaussian-density map from point annotations, and then outline the three ways \cs{to focus for free in counting} from point annotations, shown as an overview in Figure~\ref{fig:focus-overall}. \cs{Need to explain the three methods briefly? Else the reader cannot follow the figure?}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\linewidth]{figures/focus-overall.pdf}
\caption{\textbf{Overview of our approach.} 
Top: We enhance density regression by re-purposing the point annotations to develop a foreground focus with the aid of a segmentation loss $\mathcal{L}_s$ (Section \ref{sec:segmentation}) and a global density focus with the aid of a global density classification loss (Section \ref{sec:global}). Bottom: We create an auxiliary network that is trained on images with blacked-out background areas with the supervision of a Gaussian-density map, which is generated from the point annotations. Subsequently, we distill the foreground knowledge learned by the auxiliary network into the density prediction network. \psmm{Add section reference for bottom part description and choose more conventional colors. Most notably, the bright blue of "global density focus" does not fit with the other colors. I recommend choosing colors from a known color palette, see e.g. https://www.flerlagetwins.com/2021/06/datafam-colors-color-palette.html} \cs{Agree. This looks very clumsy. Certainly not IJCV-worthy.}
}
\label{fig:focus-overall}    
\end{figure*}


\subsection{Problem formulation}
\subsection{Problem formulation}
Point annotations are commonly provided as a set of coordinates $\mathcal{P}$, where each point $P{=}(x,y) \in \mathcal{P}$ indicates the location of an object in an image. From the point annotations we create a Gaussian-density map through convolutions with a normalized Gaussian kernel:
%
\begin{equation}
D(p)=\sum_{i=1}^N\mathcal{N}\big(p|\mu=P,\sigma_P^2\big),
\label{eq:density}
\end{equation}
%
where $p$ denotes a pixel location, and $\mathcal{N}(\cdot)$ is a normalized Gaussian kernel with mean $P$ and an isotropic variance $\sigma_P$. Determining $\sigma_P$ for each point $P$ is difficult because of object-size variations caused by perspective distortions. A solution is to estimate the radius $r$ of an object as a function of the $K$ nearest neighbor annotations, as done in the Geometry-Adaptive estimation of \cite{zhang2016single}. 
%However, this estimation is effective only under the assumption that objects in images are uniformly distributed, which typically does not happen in counting practice. To address this issue, we introduce an approach, which takes into account the non-uniform distribution of objects in images.
%
%\textbf{Non-uniform kernel estimation.}
%To increase the robustness of the variance estimation, we propose to estimate the size of objects locally. Specifically, we split an image into local regions and estimate the variance of a point annotation $P$ as:
%\begin{equation}
%\sigma_P = \frac{1}{|R_{(w,h)}|} \sum_{a \in R_{(w,h)}}\beta \bar{d_a}, \quad  \bar{d_a}=\frac{1}{K} \sum_{k=1}^{K}d_{k,a},
%\label{eq:sigma}
%\end{equation}
%where $w$ and $h$ are the hyper-parameters that determine the range of region $R$ centered around point annotation $P$, which we set to one-eighth of the image size in our experiments. Here, $a$ denotes an arbitrary point annotation co-located in $R$, $|R_{(w,h)}|$ denotes the number of point annotations located in $R$, $\bar{d_a}$ indicates the average distance between the annotated point $a$ and its $k$ nearest neighbors, and $\beta$ is a user-defined hyper-parameter. By estimating the variance of point annotations locally, we no longer have to assume that points are uniformly distributed over the whole image.

With both the image and the Gaussian-density map $\{(I_i,D_i)\}_{i=1}^{N}$, we optimize a deep neural network $f$ that learns to transform the images into their corresponding density maps. During inference, the global object count $T_i$ of the image $I_i$ can be obtained by simply summing all pixel values within the predicted density map, \ie, $T_i=\sum_{p \in I_i}\hat {D}_i(p)$, where $\hat {D}_i = f(I_i)$ the predicted density map.


\subsection{Foreground focus}
\label{sec:segmentation}
%Beyond creating a Gaussian-density map with point annotations, we leverage these points to establish a foreground focus, which effectively improves density map prediction.
Typically, a network for density map prediction is learned by optimizing a loss function of the form
\begin{equation}
\mathcal{L}_d{=} \ell_p(f_d(I)-D), 
\end{equation}
where $f_d$ the network, $I$ the input image, $D$ the Gaussian-density map, and $\ell_p$ the Lp norm loss function. We can reformulate the loss function by dividing the density map into two components, one representing the background of the input image and the other corresponding to the foreground containing the objects of interest:
%By dividing the density map into two components, one representing the background of the input image and the other corresponding to the foreground containing the objects of interest, we can further reformulate the loss function as $\mathcal{L}_d{=} \ell_p({f(I)}_{bg}) + \ell_p({f(I)}_{fg}-D_{fg})$,
\begin{equation}
\mathcal{L}_d{=} \ell_p({f(I)}_{bg}) + \ell_p({f(I)}_{fg}-D_{fg}),
\end{equation}
where $D_{bg}$ is naturally omitted as every single element in it is zero. Based on this reformulation, we identify two issues with current approaches. First, when $\ell_p({f(I)}_{bg})$ is not optimized perfectly, they are prone to misidentifying the background as objects (densities). Second, while trying to transform objects into densities, they cannot fully utilize their learning capacity as they predict densities by ${f(I)}_{fg}$ not only on objects but also on the background. To overcome these challenges, we propose a solution that re-purposes point annotations to create a binary segmentation map used to train a segmentation network capable of distinguishing between foreground and background areas. We then outline two approaches that leverage the segmentation masks to emphasize the foreground while suppressing the background for density prediction.

\textbf{Foreground segmentation.} We obtain a binary segmentation ground truth map $S$ as a function of the point annotations and their estimated variance. The binary value for each pixel location $p$ is determined as:
\begin{equation}
S(p) =
\begin{cases}
1 & \text{if  $\exists_{P \in \mathcal{P}} \big( ||p - P||^2 \leq \sigma_P^2$} \big),\\
0 & \text{otherwise.}
\end{cases}
\label{eq:segfocus}
\end{equation}
Equation~\ref{eq:segfocus} states that a pixel $p$ obtains a value of one if at least one point $P$ is within its variance range $\sigma_P$ as specified by a kernel estimator. By utilizing the obtained segmentation map as supervision, we train a segmentation network, $f_s$, which learns to distinguish between the foreground and background regions by optimizing a per-pixel weighted focal loss:
\begin{equation}
%\begin{split}
\mathcal{L}_s = 
 \sum_{{l} \in \{0,1\}} -\alpha{^l} S^l (1-\hat S)^{\gamma_s} log(\hat S),
\label{eq:focus-seg}
%\end{split}
\end{equation}
where $\alpha{^l}=1-\frac{|S^l|}{|S|}$ and $\hat S{=}f_s(I)$ the predicted segmentation map. The focal parameter $\gamma_s$ is set to 2 throughout this network, as recommended by \cite{lin2017focal}. 

\textbf{Focus from foreground segmentation.} One way to utilize the predicted segmentation map $f_s(I)$ is to enhance the desired foreground densities and suppress false background densities in the output density map, which we refer to as output-foreground focus.
%This approach, referred to as output-foreground focus,  was first proposed in the conference version of this work \citep{shi2019counting}.
This is done by incorporating the mask into the density prediction loss function. Specifically, through the following masked loss function
\begin{equation}
\mathcal{L}_d {=} \ell_p \big(f_d(I)\odot{f_s(I)}-D\big),
\end{equation}
where $\odot$ denotes element-wise multiplication. This approach reduces background errors and improves density prediction, but also leads to situations where densities are predicted on the background, which can hinder the transformation from objects to densities. To address this problem, we propose a second approach, referred to input-foreground focus, which simultaneously utilizes the predicted segmentation map $f_s(I)$ to highlight the desired foreground areas while suppressing false background areas in the input image. The resulting loss function becomes
\begin{equation}
\mathcal{L}_d {=} \ell_p \Big(f_d\big(I\odot {f_s(I)}\big)-D\Big).
\end{equation}
With this approach, the network only fits densities on the objects, avoiding the impact of background pixels from the start.
Input- and output-foreground focus have different trade-offs. Where input-foreground focus leads to better density prediction, output-foreground focus allows the density prediction network and the segmentation network to share the same backbone network, reducing the extra inference time required for performing additional segmentation.
%than output-foreground focus, but requires a separate segmentation network to predict the segmentation map before predicting densities. In contrast, output-foreground focus allows the density prediction network and the segmentation network to share a backbone network, reducing the extra inference time required for performing additional segmentation.

\textbf{Focus from foreground distillation.} Achieving a perfect foreground segmentation is a challenging task and any imperfections may reduce the effectiveness of the foreground focus. We propose a solution to this issue by learning how to distill true foreground knowledge. In particular, we have developed an auxiliary network that we train on images where background areas are blacked-out. The training loss is
\begin{equation}
\label{eq:auxiliary}
  \mathcal{L}_a{=} \ell_p \big({f_a(I\odot S)}-D\big),
\end{equation}
where $f_a$ is the auxiliary network, $I\odot S$ the image with background areas blacked-out, $S$ the segmentation ground truth, and $D$ the Gaussian-density map. The optimization of the auxiliary network will be stopped when it achieves maximum accuracy on the validation set. Then we distill the knowledge of the trained auxiliary network to the density prediction network with the loss
\begin{equation}
\label{eq:distillation}
  \mathcal{L}_d{=} \ell_p \big(\hat{D} - f_a(I\odot S)\big),
\end{equation}
where $\hat{D}$ represents the density map predicted with our foreground focus, which can be obtained by $f_d(I)\odot f_s(I)$ or $f_d\big(I \odot f_s(I)\big)$. Unlike traditional distillation methods that aim to compress information \citep{hinton2015distilling}, our distillation technique aims to extract foreground knowledge. In the density prediction loss function $\mathcal{L}_d$, we replace the Gaussian density map with our distilled density map for the final training, rather than do both. Foreground knowledge distillation is only performed during the training phase, hence it does not impact inference time.
%Our distillation loss is not combined with the ground truth loss because we observed that combining the two leads to a reduction in counting performance. \psmm{Previous sentence unclear, do you mean that we replace the Gaussian density map with our distilled density map for the final training, rather than do both?} 

\subsection{Global density focus}
\label{sec:global}
Aside from providing a spatial focus through foreground segmentation, point annotations can also be re-purposed to achieve a channel focus by examining contextual information through global density classification. In dense prediction tasks, it is crucial to comprehend and leverage contextual information. In the context of per-pixel density prediction for counting, global context is associated with the overall crowd density in the image. To capture such global context, we learn a global density classification task. We then utilize this captured global context to develop a channel focus that highlights feature maps that align with the global density reflected by the annotation points, leading to improved counting performance.

\textbf{Global density classification.} To perform global density classification, we first obtain a global density ground truth from the point annotation, for free. Specifically, the global density for a patch $j$ in the training image $i$ is given as:
\begin{equation}
G_{j,i} = \frac{|\mathcal{P}_{j,i}|}{L}, L = \left \lfloor{ \max_{i=1,..,N} \Big (\frac{|\mathcal{P}_{i}|}{Z_i} \cdot Z_{j,i}\Big) / M}\right \rfloor + 1.
\end{equation}
Here $|\mathcal{P}_{j,i}|$ denotes the number of object points in patch $j$, $L$ denotes the global density step size, $Z_i$ and $Z_{j,i}$ denote the number of pixels in image $i$ and patch $j$ respectively. The step size calculation involves determining the highest global density across image patches, while the parameter $M$ denotes the number of global density levels used in the process. By leveraging the global density ground truth, we train a network $f_c$ for classifying global density with the following loss:
\begin{equation}
\mathcal{L}_c = 
\sum_{{l} \in \{0,1,..,M\}} -G^l (1-\hat G)^{\gamma_c} log(\hat G),
\label{eq:global density}
\end{equation}
where $\hat G{=}f_c(I)$ and $\gamma_c$ is set to 2. The $f_c$ model comprises a backbone network and a classifier. The backbone network is shared with the per-pixel density prediction network $f_d$. To capture feature statistics in a global context, we incorporate a global average pooling on top of the backbone network. The classifier comprises two fully-connected layers and a softmax function. 

%\textbf{Focus from global density classification.} 
After capturing the global context, we develop a channel focus that emphasizes feature maps aligned with the global density. To achieve this, we employ two fully-connected layers followed by a sigmoid function on top of the bilinear pooling layer, which generates a global density focus output. The resulting focus output is then utilized by the density prediction network's backbone to highlight feature maps that exhibit similar global contextual patterns to the ground truth density maps. %This leads to enhanced counting results.
%\psmm{explain here how global context is embedded in overall framework, i.e. how is it linked with the density estimation?}

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/global_density.pdf}
\caption{\textbf{Global density focus.} Bilinear pooling extracts essential global context information. Then two distinct branches process the resulting context. The top branch, consisting of an MLP and a sigmoid function, generates a focus map that highlights important feature maps. The bottom branch, comprising an MLP and a Softmax function, enhances the extracted context by learning to classify global density. \psmm{Match colors with updated Figure 1}}
\label{fig:segmentation}    
\end{figure}


\begin{figure}[t!]
\centering
\begin{subfigure}{\linewidth}
\includegraphics[width=\textwidth]{figures/occlusion_density.pdf}
\caption{\textbf{Occlusion simulation for point annotations}}
\label{fig:augmentation-a}    
\end{subfigure}
\begin{subfigure}{\linewidth}
\includegraphics[width=\textwidth]{figures/occlusion_image.pdf}
\caption{\textbf{Occlusion simulation for image}}
\label{fig:augmentation-b}    
\end{subfigure}
\caption{\textbf{Occlusion simulation.} (a): We randomly choose two object points from an object point map, one for the object which will be occluded, denoted by $\mathcal{O}_{occ}$ and another for the object which will be copied and pasted, denoted by $\mathcal{O}_{copy}$. The pasted position of $\mathcal{O}_{copy}$ is computed based on Eq. (\ref{eq:occlusion}), as indicated by $\mathcal{O}_{paste}$.
%
(b): We generate an occluded image  from $\mathcal{O}_{occ}$, $\mathcal{O}_{copy}$, and $\mathcal{O}_{paste}$. To avoid boundary artifacts, we perform blending to smooth out the boundary artifacts. \psmm{Match colors with updated Figure 1}
}
\label{fig:cases}    
\end{figure}


\subsection{Focus by simulating occlusion}
\label{sec:occlusion}
Finally, we utilize annotation points to augment overlapping objects to overcome the occlusion challenge. Occlusions often happen in congested scenes, resulting in overlapping objects. For counting purposes, one  solution to handle various occlusion levels is to learn a network with sufficient number of training samples for each occlusion level. However, the occlusion level presents a long-tailed distribution in all benchmarks  \citep{zhang2016single,idrees2018composition,sindagi2020jhu-crowd++,guerrero2015extremely}. In other words, there are simply not enough images in current datasets to properly learn from natural occlusions. As a remedy, we propose to simulate various occlusion levels through augmentation.

\textbf{Occlusion simulation.} 
Given a training sample consisting of an input image and its point annotations, $(I, {P_i}{i=1}^{N})$, we represent any object $\mathcal{O}_i$ in the image $I$ as $(x_i,y_i,2\sigma_i)$. Here, $(x_i, y_i)$ represents the coordinate of the corresponding annotated point $P_i$, and $\sigma_i$ is the variance of the corresponding Gaussian kernel. This representation assumes that the object $\mathcal{O}_i$ is circular and its radius is approximately equal to $2\sigma_i$, as proposed in~\cite{lempitsky2010learning}. To generate occlusion scenarios, we randomly select an object, $\mathcal{O}{occ}$, to be occluded. We then select one of its neighboring objects, denoted as $\mathcal{O}{copy}$, which will be copied and pasted to occlude $\mathcal{O}{occ}$. The pasted position of $\mathcal{O}{copy}$ determines how $\mathcal{O}_{occ}$ will be occluded, defined as: 
%
\begin{equation}
  \begin{aligned}
  x_{paste} &= \lfloor r \cdot cos(\theta) \rfloor + x_{occ},\\
  y_{paste} &= \lfloor r \cdot sin(\theta) \rfloor + y_{occ},
  \end{aligned}
  \label{eq:occlusion}
\end{equation}
%
where $r{=}r_{copy}+r_{occ} \epsilon_r$ and $\theta {=} 2\pi \epsilon_{\theta}$. $\epsilon_r$ and $\epsilon_{\theta}$ are randomly sampled from $\mathcal{U}(0,1)$. $\lfloor \cdot \rfloor$ is the floor operator. $r$ and $\theta$ decide how much and where $\mathcal{O}_{occ}$ will be occluded. 

\textbf{Blending.} Directly pasting objects on an image creates boundary artifacts, which may affect the network's learning ability. To handle boundary artifacts, we perform blending to smooth out the boundary artifacts. Specifically, we first copy and paste the object $\mathcal{O}_{copy}$ to the position $(x_{paste},y_{paste})$ of the image $I$, generating a new image $\hat I$. Then, we compute the binary mask $\alpha$ of the pasted object $\mathcal{O}_{paste}$, which we represent by $(x_{paste},y_{paste},r_{paste})$ where $r_{paste}{=}r_{copy}$. To smooth out the edges of the pasted object, we apply a Gaussian filter to the binary mask $\alpha$ and obtain a smoothed mask $\tilde \alpha$. From $\tilde \alpha$ we construct the occluded image $I_{occ}$ and its corresponding ground truth density map:
%
\begin{equation}
  \begin{aligned}
  I_{occ} &= (1-\tilde \alpha)\odot I + \tilde \alpha \odot \hat I,\\
  D_{occ} &= D + G(\mathcal{O}_{paste}),
  \end{aligned}
  \label{eq:blending}
\end{equation}
%
where $D$ denotes the ground truth density map of the image $I$, $G(\mathcal{O}_{paste})$ denotes the density map of the pasted object $\mathcal{O}_{paste}$, and $G$ denotes the Gaussian kernel. Equation \ref{eq:blending} states that the pixels to be occluded in the original image are replaced by the pixels of the pasted object to obtain the occluded image. The corresponding occluded density map is obtained by simply adding the density map of the pasted object to the original density map. 

\textbf{Occluding adaptively.} For a training image, we need to decide how many of its objects will be occluded with our approach. A simple way is to set a fixed ratio. However, the training image may already have naturally occluded objects. Thus, we should create new occlusion for the training image according to its current occlusion level. Intuitively, the lower the occlusion level, the higher the amount of occlusions that should be simulated. To compute the occlusion level, we create an occlusion map $M$ for the training image by,
% 
\begin{equation}
\begin{aligned}
&M(x,y) = \sum_{i=1}^N S(x,y;\mathcal{O}_i), \text{where} \\ &S(x,y;\mathcal{O}_i) = \mathds{1}(||x - x_i||^2 + ||y - y_i||^2 \leq (r_{i})^2). 
\end{aligned} 
\label{eq:occmap} 
\end{equation}
%
Here $(x,y)$ denotes a pixel location, $\mathcal{O}_i{=}(x_i,y_i,r_{i})$ denotes an object, and $\mathds{1}(\cdot)$ is a binary indicator function, which states that a pixel obtains a value of one if it is within an object region. Hence, each pixel value in the occlusion map $M$ indicates the amount of object regions it belongs to. The occlusion level $\bar M$ is computed as the average value of non-zero pixels in the occlusion map $M$. Then the percentage of the objects to be occluded can be adaptively obtained by $\beta $/$\bar M$ where $\beta$ is the upper boundary, and $\beta{=}0.3$ empirically performs well.

\subsection{Transformer with focus-for-free}
\label{sec:transformer}

\cs{Need to discuss structure of section 3, I get a bit confused by all the bells and whistles that are introduced and how they are related. I did not see this transformer in Figure 1. How related? Also, what is new? Isn't it just implementation details?}

Transformer architectures have shown significant promise in  counting and is quickly becoming the preferred backbone. As a result, we are inspired to incorporate our foreground focus and global density focus in transformers and leverage their capabilities to further advances counting models.

\textbf{Token-to-token Encoder.} Instead of relying on the basic tokenization approach employed in Vit \citep{dosovitskiy2020image}, we adopt the progressive tokenization module introduced by \cite{yuan2021tokens}. This module enables us to aggregate adjacent tokens into a single token, thereby incorporating local structural information from surrounding tokens and reducing the token length in a step-by-step manner. To be more specific, we utilize a Token-to-Token (T2T) mechanism, where tokens produced by a transformer layer are first reconstructed as an image, then split into overlapping patches, and finally aggregated by flattening the patches. This process allows the local structure of surrounding patches to be embedded into the tokens, which are subsequently fed into the next transformer layer. By performing T2T iteratively, the local structure is integrated into the tokens, and the token length is reduced via the aggregation process. Finally, we use an efficient deep-narrow backbone structure for the vision transformer to learn the representations from these tokens. 

\textbf{Foreground focus decoder.} To design the decoder for foreground focus, we have adopted a multi-level feature aggregation approach inspired by the feature pyramid network \cite{kirillov2019panoptic}. However, instead of using a pyramid shape, we leverage the feature representations from different layers of the T2T-Vit encoder, which have the same resolution. We begin by selecting $m$ layers from the encoder, uniformly distributed across the layers with a step of $n$. We then deploy $m$ streams, each focusing on one specific selected layer. In each stream, we first reshape the encoder's feature $Z^l$ from a 2D shape to a 3D feature map. Next, we apply a 3-layer convolutional network to process the feature from each stream. To promote interactions across different streams, we introduce a top-down aggregation design through element-wise addition after the first layer. An additional $3\times3$ convolution layer is applied after the element-wise auditioned feature. After the third layer, we obtain the fused feature from all the streams via channel-wise concatenation. This feature is then upsampled $2\times$ to match the resolution of the output density map.

\textbf{Global density focus decoder.} To capture global context information and improve it using a global density classification loss, we employ a bilinear pooling when CNN is used as encoder. However, when using a vision transformer as the encoder, we assign the task of capturing global context to a global density class token.
we use the global density class token to predict global density. To achieve this, two fully-connected layers with Softmax activation is utilized. Additionally, this token serves as the primary input to the global density focus module, which consists of two fully-connected layers with a Sigmoid activation. The global density focus module's objective is to refine the local feature map used for crowd density map prediction, given the global density class token. By doing so, the network can focus on critical feature channels, resulting in improved features.

\psmm{Maybe a figure with the overall new transformer architecture is helpful? to discuss}



%The first one involves generating foreground masks from the point annotations. Then we use the foreground masks to train a segmentation network for learning to predict the foreground of the input images, and train an auxiliary network for learning how to distill true foreground knowledge in Section~\ref{sec:segmentation}. \psmm{First novel part is not written clearly. The first sentence is that we create segmentations, which we did before already. Make very clear what is new here in easy words.} Current approaches employ segmentation maps to enhance the desired foreground densities and suppress false background densities in the output density map, \eg, ~\cite{modolo2021understanding,shi2019counting,qian2022segmentation,zhao2019leveraging}. However, confusion with the background of the input images contributes to over half of the error rate across approaches and datasets (as demonstrated in an oracle experiment in Section~\ref{sec:exp_segmentation}). Therefore, the key to better counting is to avoid counting on background pixels altogether. To reduce the impact of counting on the background, we cascade a segmentation and density network. Nonetheless, achieving perfect foreground segmentation is challenging, and any imperfections may diminish the effectiveness of the foreground focus. To address this issue, we propose a solution by learning how to distill true foreground knowledge.
%\psmm{There is a lot of text above, but I don't know what is old and what is new. No need to fully explain what is going on yet, focus on what we propose and what is new, keep it short.}
%The second one involves explicitly simulating counting-specific occlusions with point annotations. Congested scenes with high levels of occlusion are common in counting, but occlusions rarely appear in training imagery, hindering the network's ability to handle occlusions properly. In Section~\ref{sec:occlusion}, we demonstrate that occlusions can be simulated through augmentation on both the input image and density maps. Overall, we make three contributions in this paper:

%Summarized, we make the following contributions:
%\begin{itemize}
%  \item We introduce foreground focus and distillation, which involves generating foreground masks from point annotations. This approach is effective in limiting the impact of background pixels on counting accuracy.
%  \item We propose a counting-specific augmentation technique that utilizes point annotations on both input and density images to enhance the network's robustness to occlusions.
%  \item We integrate the aforementioned techniques and global density focus proposed in \cite{shi2019counting} into modern counting networks such as convolutional neural networks and vision transformers. This amalgamation of methods enables our networks to accurately count objects of interest even in challenging scenarios, such as background clutter, occlusion, and varying crowd densities.
%\end{itemize}
%\psmm{If paragraph above is written well, this itemize is no longer needed.}

==> temp1.tex <==
\section{Experiments and results}
We first describe the experimental setup. We then analyze the effect of three types of focuses proposed in this work, comparing each to their respective baseline approaches. Finally, we report the results of the combination of the three focuses and compare them to the state-of-the-art.
%===============================
\subsection{Experimental setup}
%===============================
\textbf{Datsets.}  We consider five counting datasets in this paper commonly used in the recent literature, \eg,~\citep{bai2020adaptive,wan2021generalized,liu2021exploiting,wang2021uniformity,song2021rethinking,ma2021towards}:
%
\textbf{\textit{ShanghaiTech}} \citep{zhang2016single} consists of 1,198 images with 330,165 pedestrians. This dataset is divided into two parts: \textbf{\textit{Part\_A}} with 482 images in which crowds are mostly dense, and \textbf{\textit{Part\_B}} with 716 images, where crowds are sparser. Each part is divided into a training and testing subset as specified in \citep{zhang2016single}. 
%
\textbf{\textit{UCF-QNRF}} \citep{idrees2018composition} consists of 1,535 images, with the count ranging from 49 to 12,865. 
For training 1,201 images are available, the remaining 334 form the test set. 
%
\textbf{\textit{JHU-CROWD++}} \citep{sindagi2020jhu-crowd++} consists of 4,372 images with a total of 1.51 million point annotations. 
The dataset is split into a training set of 2,272 images, a validation set of 500 images and a testing set of 1,600 images.
\textbf{\textit{NWPU-Crowd}} \citep{wang2020nwpu} consists of 5,109 images with over 2 million point annotations. 
The dataset is split into a training set of 3,109 images, a validation set of 500 images and a testing set of 1,500 images. 

For all datasets, we augment the images by randomly performing horizontal flipping, and randomly cropping $256 {\times} 256$ patches for ShanghaiTech, JHU-CROWD++ and $416 {\times} 416$ patches for UCF-QNRF, NWPU. For Gaussian density map generation, we follow the previously suggested dataset settings from \citep{zhang2016single,idrees2018composition,sindagi2020jhu-crowd++}.

\textbf{Network.} We have adopted CSRNet \citep{Li_2018_CVPR} as the convolutional base network for our counting task. CSRNet is a widely-used architecture in the literature, as evidenced by its use in several studies \citep{zhao2019leveraging,ma2019bayesian,wan2020modeling,wang2020distribution,wan2021generalized,ma2021towards}. To improve its performance, we have followed the lead of \cite{bai2020adaptive} and incorporated batch normalization layers into our implementation of CSRNet, which refers to CSRNet+. To integrate our focuses with CSRNet+, we have used the architecture presented in Fig. \ref{fig:focus-overall} Specifically, we have used the same backbone network as the frontend network of CSRNet+, and the same output-foreground focus module and density regressor module as the backend network of CSRNet+.  To implement our output-foreground focus, we use HRNetv2-W48 \citep{wang2020deep} as the segmentation network throughout this paper.
In addition to CSRNet+, we have also utilized the T2T-ViT-14 \citep{yuan2021tokens} as the vision transformer base network. We have followed the instructions presented in section \ref{sec:transformer} to incorporate our focuses into this network as well.

\textbf{Optimization.} Both networks have been initialized with their ImageNet pre-trained models and trained using Adam with batches of 10. By default, we have used an $\ell_1$ loss function. The learning rate has been fixed at 1e-4 for CSRNet+ and le-5 for T2T-ViT-14.

\textbf{Metrics.} We report the standardized Mean Absolute Error (MAE) and Root Mean Square Error (RMSE) metrics given count estimates and their ground-truth.
%
\begin{table}[!t]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}lcccccccccccccccc@{}}
\toprule
& \multicolumn{2}{c}{\textbf{CSRNet+}} &
\multicolumn{2}{c}{\textbf{T2T-Vit}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& \textit{Part\_A} & \textit{UCF\_QNRF} & \textit{Part\_A} & \textit{UCF\_QNRF}\\
\hline
Standard  &61.9 &117.6 & 60.1 &89.8\\
w/o BG in output density &53.6 &81.4 &51.6 &80.7\\
\rowcolor{Gray}
w/o BG in input image &29.8 &32.4 &27.7 &54.6\\
\bottomrule
\end{tabular}}
\caption{\textbf{Impact of background error.} Removing the background pixels with an oracle before density prediction reduces the count error (MAE) considerably across datasets and networks.}
\label{tab:seg}
\end{table}
%
%
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{}lccccccccccccccc@{}}
\toprule
& \multicolumn{6}{c}{\textbf{\textbf{CSRNet+}}} & \multicolumn{6}{c}{\textbf{\textbf{T2T-Vit}}}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} & \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
& \textit{BG}  & \textit{FG}  & \textit{Overall} & \textit{BG} & \textit{FG} & \textit{Overall} & \textit{BG}  & \textit{FG}  & \textit{Overall} & \textit{BG} & \textit{FG} & \textit{Overall} \\
\hline
Base network & 3.4 & 61.5 & 61.9 &8.7 & 91.3 &93.6 & 3.2 & 59.1 & 60.1 &8.2 & 89.9 &90.4\\
w/ background feature filtering \citep{mo2020background} & 3.1 & 58.2 & 58.8 &4.3 & 87.1 &88.3 &2.9 & 57.1 &57.7 &4.8 & 87.6 &87.9 \\
w/ attention-injective \citep{liu2019adcrowdnet} & 3.3 & 59.7 & 60.5 &6.1 & 89.9 &91.2 & 3.0 & 58.5 &59.1 &5.8 & 89.1 &89.8\\
w/ decoupled learning \citep{cheng2021decoupled} & 3.1 & 57.1 & 57.5 &3.5 &84.8 &85.6 &2.9 & 55.8 &56.7 &\textbf{4.1} & 83.6 &84.2\\
\hline
w/ our output-foreground focus \citep{shi2019counting} & 3.2 & 59.1 & 59.6 &5.2 & 89.6 &90.3 & 3.1 & 58.2 &58.5 &4.9 & 89.4 &89.1 \\
\rowcolor{Gray}
w/ our input-foreground focus & \textbf{3.0} & \textbf{55.3}&\textbf{56.1}&\textbf{3.4}& \textbf{83.6} &\textbf{84.4} &2.9& \textbf{54.2} &\textbf{55.4} &4.8 &\textbf{82.7} &\textbf{83.6}\\
\bottomrule
\end{tabular}
\end{threeparttable}}
\caption{\textbf{Effect of foreground focus.} Compared to base networks and our reimplementation of four related works, which predict density maps on the background, our simple cascade model with background reduction reduces the overall count error (MAE), for both background (BG) and foreground (FG).  
}
\label{tab:seg+dis}
\end{table*}
%
%
\begin{figure*}[t!]
\centering
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/cascade/cascade_input.pdf}
\caption{\textbf{Input image}}
\label{fig:segmentation-a}    
\end{subfigure}
\begin{subfigure}{0.245\textwidth}
\includegraphics[width=\textwidth]{figures/cascade/cascade_seg.pdf}
\caption{\textbf{Cascaded image}}
\label{fig:segmentation-b}    
\end{subfigure}
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/cascade/cascade_density.pdf}
\caption{\textbf{Our density}}
\label{fig:segmentation-c}    
\end{subfigure}
\begin{subfigure}{0.243\textwidth}
\includegraphics[width=\textwidth]{figures/cascade/cascade_gt.pdf}
\caption{\textbf{Ground-truth}}
\label{fig:segmentation-d}    
\end{subfigure}
\caption{\textbf{Learning to avoid the background.}  Segmentation and density prediction results by our cascade model. While by no means perfect, the predicted segmentation masks already reduce the background pixels considerably. The density prediction network is then able to count correctly on the remaining amount of background pixels, as masked in the green regions. }
\label{fig:segmentation}    
\end{figure*}
%===============================
\subsection{Foreground focus}
\label{sec:exp_segmentation}
%===============================
\textbf{Impact of background interference.}
In section \ref{sec:segmentation}, we introduce two foreground focus techniques that aim to reduce the impact of background interference in output density maps or input images. Before evaluating the effectiveness of these methods, we need to quantify how much the background impedes counting performance. To accomplish this, we use oracle segmentation maps based on Eq. \ref{eq:segfocus}. To examine the background error in the output density map, we apply the oracle segmentation map to mask the output density map predicted by the baseline counting network from the input image. Alternatively, we use the oracle segmentation map to mask the input image itself and then apply the baseline counting network to the masked image to predict the density map. It's worth noting that the original input image and its background-free equivalent share the same ground-truth density map.

Table~\ref{tab:seg} presents the results of our experiments on two counting networks and two datasets. The results consistently show that removing the background from either the input image or the output density significantly reduces MAE. Although removing the background from the output density reduces background errors, the density maps are still predicted with the input image's background. On the other hand, removing the background from the input image eliminates background errors in the output density and prevents the prediction of densities on the background. Our experiments demonstrate that by predicting the density maps without the background, the counting error can be significantly reduced. For instance, on the ShanghaiTech Part\_A dataset, CSRNet+ reduces the MAE from 61.9 to 53.2 by removing the background error from the output density but achieves a much lower MAE of 29.8 by predicting the density maps without the background. This result surpasses the current state-of-the-art on this dataset by a considerable margin. Our findings suggest that the interference caused by the input image's background could be responsible for most of the counting error. In conclusion, our oracle experiment highlights that removing the background from the input image can significantly enhance density-based counting.

\textbf{Effect of focus from foreground segmentation.}
Motivated by the oracle experiment, our counting model with input-foreground focus cascades a segmentation network and a density prediction network to reduce the impact of background pixels from the start. To emphasize that the key is to remove the background from the input image altogether, we compare it to the other four baselines. The first one \citep{mo2020background} filters the background noise on the intermediate features by learning a head segmentation mask. The second baseline \cite{liu2019adcrowdnet} is a cascade counting approach, which cascades a crowd-level attention prediction network and a density estimation network.
%
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{cccccccccccc}
\toprule
\multicolumn{3}{c}{\textbf{Foreground focus}} & \multicolumn{2}{c}{\textbf{CSRNet+}}&\multicolumn{2}{c}{\textbf{T2T-Vit}} \\
\cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Foreground distillation &Output-foreground focus & Input-foreground focus  &\textbf{Part\_A} & \textbf{UCF\_QNRF} &\textbf{Part\_A} & \textbf{UCF\_QNRF}  \\
\hline
 & & & 61.9 & 117.6&60.1 &89.8 \\
\rowcolor{Gray}
 \checkmark& & &58.7&103.3&- &-\\
  &\checkmark& & 59.6&92.8&- &-\\
\rowcolor{Gray}
\checkmark&\checkmark& &55.4&87.2&-&-\\
  & &\checkmark&57.8&-&-&-\\
\rowcolor{Gray}
 \checkmark& &\checkmark  &54.9&-&-&-\\

\bottomrule
\end{tabular}
\end{threeparttable}}
\caption{\textbf{Effect of foreground distillation.} Foreground distillation significantly improves the performance when used directly with the base network, or in conjunction with output-foreground focus or in-foreground focus.}
\label{tab:seg+dis}
\end{table*}
%
%
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{}lccccccccccccccc@{}}
\toprule
& \multicolumn{6}{c}{\textbf{\textbf{CSRNet+}}} & \multicolumn{6}{c}{\textbf{\textbf{T2T-Vit}}}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} & \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
& \textit{sparse}  & \textit{dense}  & \textit{Overall} & \textit{sparse}  & \textit{dense}  & \textit{Overall} & \textit{sparse}  & \textit{dense}  & \textit{Overall} & \textit{sparse}  & \textit{dense}  & \textit{Overall} \\
\hline
Base network & 35.8 & 88.0 &61.9 &- & - &- &37.4 &82.8 &60.1 &- &- &-\\
w/ CBAM \citep{woo2018cbam} &36.5 &85.9 &61.2 &- & - &- &36.8 &82.6 &59.7 &- &- &-\\
w/ SE \citep{hu2018squeeze} & 36.9 &84.3 & 60.6 &- & - &- &36.1 &82.7 &59.4 &- &- &-\\
\rowcolor{Gray}
w/ our global density focus& 35.0 & 83.2 & 59.1 &- & - &- &35.5 &81.9 &58.7 &- &- &-\\
\bottomrule
\end{tabular}
\end{threeparttable}}
\caption{\textbf{Effect of global density focus.} Our approach, which incorporates explicit supervision for channel attention, outperforms both the base networks and two related works that implement channel attention implicitly. Our method significantly reduces the mean absolute error (MAE) for both sparse and dense crowd counting. 
}
\label{tab:gf}
\end{table*}
%
The third baseline \cite{cheng2021decoupled} learns to count with decoupled learning, which first regresses a probability map to identify possible object regions, and then predicts a density map on the probability map to count the objects. The last baseline is our previous output-foreground focus \citep{shi2019counting}. As shown in Table~\ref{tab:seg+dis}, all four baselines perform better than the base network only, while our method even better improves both background and foreground errors, with a special focus on the foreground error. With the CSRNet+ base network, for instance,  on ShanghaiTech Part\_A our approach provides a reduction of 5.8 in the overall MAE. On UCF \_QNRF, the overall MAE even goes down by 9.2. The results emphasize the importance of removing the background in the input image for counting. We also provide qualitative results in Figure \ref{fig:segmentation}. We observe that our predicted segmentation masks remove many background pixels, and the density prediction network is able to count well on the remaining pixels. 
%
Overall, we recommend learning to remove the background from the input image for density-based counting. The gap towards oracle performance further highlight that big gains should be feasible with more advanced image segmentation.

\textbf{Effect of foreground distillation.}
%We propose a novel technique called foreground distillation, aimed at bridging the performance gap between oracle segmentation and learned segmentation. Our method involves utilizing the same base network for both auxiliary distillation and density prediction.
We have conducted experiments to evaluate the effectiveness of our proposed foreground distillation when used directly with the base network, or in conjunction with output-foreground focus or in-foreground focus. Our results, shown in Table~\ref{tab:seg+dis}, indicate that foreground distillation significantly improves the performance in all three scenarios. For example, using the base network CSRNet+ alone, our approach reduces MAE by 3.2 on ShanghaiTech Part\_A. With the addition of output-foreground focus or input-foreground focus, the MAE further goes down by 4.5 or 5.8, respectively. Foreground distillation is a simple yet effective approach that can be easily applied to any network, resulting in a direct reduction in counting errors. 
%
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.99\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{}lccccccccccccccc@{}}
\toprule
& \multicolumn{6}{c}{\textbf{\textbf{CSRNet+}}} & \multicolumn{6}{c}{\textbf{\textbf{T2T-Vit}}}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} & \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
& \textit{Low}  & \textit{High} &\textit{Overall}  & \textit{Low}  & \textit{High} & \textit{Overall}& \textit{Low}  & \textit{Dense} &\textit{High}  & \textit{Low}  & \textit{Dense} & \textit{High} \\
\hline
Base network & 39.2 & 95.9 & 61.9 &18.7& 106.5 &93.6 & 36.5 & 94.3 & 59.7 &17.2& 103.0 &90.4\\
w/ cutout \citep{devries2017cutout} & 38.6 & 95.0 & 61.2 &\textbf{16.5}& 104.7 &91.8 & 35.6 & 93.5 & 58.8 &\textbf{15.4}&101.5 &88.5\\
w/ cutmix \citep{yun2019cutmix} &38.0 & 94.3 &60.6 &17.8&103.1 &90.6 & 35.2 & 92.8 & 58.3 &16.3&99.8&87.6\\
\rowcolor{Gray}
w/ ours  &\textbf{37.8} & \textbf{91.2} &\textbf{59.1} &18.3& \textbf{99.3} &\textbf{87.4} &\textbf{34.7} & \textbf{90.5} & \textbf{57.1} &16.8& \textbf{98.1} &\textbf{86.2}\\
\bottomrule
\end{tabular}
\end{threeparttable}}
\caption{\textbf{Effect of our solution for occlusion error.} Compared to a base network and our reimplementation of two related works, our occlusion augmentation reduces the count error (MAE) for the entire test set, the \emph{low} occlusion set, and especially for the \emph{high} occlusion set. 
}
\label{tab:occlusion}
\end{table*}
%
%
\begin{figure*}[!t]
\centering
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/occ/img_ori.pdf}
\caption{\textbf{Original image}}
\label{fig:augmentation-a}    
\end{subfigure}
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/occ/img_ours.pdf}
\caption{\textbf{Our image}}
\label{fig:augmentation-b}    
\end{subfigure}
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/occ/den_ori.pdf}
\caption{\textbf{Original density}}
\label{fig:augmentation-c}    
\end{subfigure}
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/occ/den_ours.pdf}
\caption{\textbf{Our density}}
\label{fig:augmentation-d}    
\end{subfigure}
\caption{\textbf{Occlusion creation}. Illustrative examples for creating new occlusions on images and corresponding density maps. Our occlusion-augmented image and density look quite natural, as masked in the green regions.}
\label{fig:augmentation}   
\end{figure*}
%===============================
\subsection{Global density focus}
%===============================
Next, we demonstrate the effect of our proposed global density focus module. We compare it with the SE module \citep{hu2018squeeze} and the channel attention module of CBAM \citep{woo2018cbam}, while keeping the base network unchanged. To ensure a fair comparison, we use the same MLP network for all the approaches.

To evaluate the performance of our module, we define the crowding level of each image as $I_{crowd} = \frac{N(\mathcal{O})}{S(I)}$, where $N(\mathcal{O})$ represents the number of objects in the image, and $S(I)$ denotes the size of the image. We then sort the test images in ascending order based on their global density level and divide them uniformly into three sets: sparse, medium, and dense. By doing so, we demonstrate that our module exhibits a lower error on different crowding levels.

The results of our experiment are presented in Table \ref{tab:gf}. Both SE and CBAM can already improve the base network's performance based on both CSRNet+ and T2T-Vit. Our proposed global density focus outperforms SE and CBAM, reducing the count error even further, due to its explicit supervision. 
%
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multicolumn{3}{c}{\textbf{Three ways of focus by repurposing point annotations}} & \multicolumn{2}{c}{\textbf{CSRNet+}}&\multicolumn{2}{c}{\textbf{T2T-Vit}} \\
\cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Foreground focus & Global density focus & focus by simulation &\textbf{Part\_A} & \textbf{UCF\_QNRF} &\textbf{Part\_A} & \textbf{UCF\_QNRF}  \\
\hline
 & & & 61.9 & 93.6&59.7 &90.4 \\
 \checkmark & & & 56.1&84.4&55.4 &83.6\\
 \checkmark&\checkmark &  &54.7 &82.2&53.4 &81.5\\
\checkmark& & \checkmark & 53.5 &81.2&51.2 &79.6\\
\rowcolor{Gray}
\checkmark&\checkmark & \checkmark & \textbf{52.4} & \textbf{79.8}& \textbf{49.1} & \textbf{78.2}\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Effect of combining our three focus solution} in terms of MAE on ShanghaiTech Part\_A and UCF\_QNRF. With each new addition, the counting error decreases, showing their complementary nature.}
\label{tab:combine}
\end{table*}
%
\begin{table*}[t!]
\centering
\resizebox{0.99 \linewidth}{!}{
\begin{tabular}{@{}lccccccccccccr@{}}
\toprule
&\multirow{2}{*}{\textbf{Backbone}} &\multicolumn{2}{c}{\textbf{Part\_A}} & \multicolumn{2}{c}{\textbf{Part\_B}}&\multicolumn{2}{c}{\textbf{UCF\_QNRF}}&\multicolumn{2}{c}{\textbf{JHU-CROWD++}}&\multicolumn{2}{c}{\textbf{NWPU-Crowd}}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}  \cmidrule(lr){11-12}
 & & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE &  RMSE\\
\hline
\rowcolor{Gray} 
\textbf{Lp loss}&&&&&&&&&&&&\\
\cite{xu2022autoscale} &VGG-16&65.8 &112.1 &8.6 &13.9 &104.4 &174.2 &76.4&292.7&94.1&388.2\\
%
\cite{wan2020kernel} &VGG-16&63.8 &99.2 &7.8 &12.7 &99.5 &173.0 &69.7&268.3&100.5&415.5\\
% 
\cite{ma2021towards} &VGG-16&58.4 &97.9 &- &- &96.3&155.7 &65.1&269.3 &- &-\\
\cite{shu2022crowd} &VGG19&57.5&94.3 &6.9 &11.0 &80.3 &137.6 &57.0 &235.7 &76.8 &343.0 \\
%
\cite{cheng2021decoupled} &VGG-16&57.2 &93.0 &6.3 &10.7 &81.7&137.9 &73.7&292.5 &85.5 &361.5\\
%
\cite{bai2020adaptive} &VGG-16&55.4 &97.7 &6.4 &11.3 &\underline{\textbf{71.3}}&&- &- &- &-\\
%
\cite{tran2022improving} &ViT-B/32&54.8 &80.9 &8.6 &13.8 &87.0&141.9 &-&- &- &-\\
%
\cite{cheng2022rethinking} &ResNet-50&54.8 &89.1 &6.2 &9.9 &81.6&153.7 &58.2&245.1 &- &-\\
%
\cite{wang2021uniformity} &VGG-16&54.6 &91.2 &6.4 &10.9 &81.1&131.7 &-&- &- &-\\
%
\textit{\textbf{Ours (CSRNet+)}} &VGG-16&- &- &- &- &-&- &-&- &- &-\\
%
\textit{\textbf{Ours (T2T-Vit)}} &T2T-Vit-14&\underline{\textbf{49.1}} &\underline{\textbf{83.2}} &\underline{\textbf{6.1}} &10.3 &78.2& \textbf{126.5} &\underline{\textbf{56.8}}&253.4 &\underline{\textbf{-}} &\underline{\textbf{-}}\\
%
\midrule
\rowcolor{Gray} 
\textbf{DM loss}&&&&&&&&&&&&\\
%
\cite{wan2021generalized} &VGG19&61.3 &95.4 &7.3 &11.7 &84.3&147.5 &59.9&259.5 &79.3 &346.1\\
%
\cite{wang2020distribution}  &VGG-19&59.7 &95.7 &7.4 &11.8 &85.6 &148.3 &- &- &88.4 &388.6 \\
%
\cite{liu2021exploiting} &ResNet-18&55.4 &91.3 &6.9 &10.3 &76.2&\underline{121.5} &59.9&259.5 &\underline{74.7} &\underline{267.9}\\
%
\cite{ma2021towards} &VGG-19&55.0 &92.7 &- &- &80.7&146.3 &59.3&\underline{\textbf{248.9}} &- &-\\
%
\cite{sun2021boosting} &T2T-Vit-14&53.1 &82.2 &7.3 &11.5 &83.8&143.4 &54.8&208.5 &82.0 &366.9\\
%
\cite{song2021rethinking} &VGG-16&52.7 &85.1 &6.3 &\underline{9.9} &85.3&154.5 &-&- &77.4 &362.0\\
%
\textit{\textbf{Ours (CSRNet+)}} &VGG16&- &- &- &- &-&- &-&- &- &-\\
%
\textit{\textbf{Ours (T2T-Vit)}} &T2T-Vit-14&\underline{\textbf{-}} &\underline{\textbf{-}} &\underline{\textbf{-}} &- &-& \textbf{-} &\underline{\textbf{-}}&- &\underline{\textbf{-}} &\underline{\textbf{-}}\\

\bottomrule
\end{tabular}}
\caption{\textbf{Comparison to the state-of-the-art} on ShanghaiTech Part\_A, Part\_B, UCF\_QNRF, JHU-CROWD++ and TRANCOS.
%Our results set a new state-of-the-art on most datasets for most metrics.
We combine our three solutions with CSRNet+ and T2T-Vit to obtain counting results which are either competitive or better than the current state-of-the-art, highlighting their potential for density-based counting. \textbf{Bold} indicates the best density-based counting results, and \underline{underline} indicates the best overall counting approach.}
\label{tab:sota}
\end{table*}
%
%===============================
\subsection{Focus by simulating occlusion}
%===============================
In this experiment, we demonstrate the potential of our occlusion handling augmentation. To highlight effectiveness in highly occluded images, we divide the test images into two sets according to their occlusion level, as computed by Equation \ref{eq:occmap}. The test images are grouped into the \emph{low} occlusion set if their occlusion level is lower than $1.5$, the remaining images are grouped into the \emph{high} occlusion set. For ShanghaiTech Part\_A, we obtain 109 low and 73 high occlusion images and for UCF\_QNRF, we obtain 49 low and 285 high occlusion images. To highlight that the key here is occlusions, not just the augmentation, we have additionally investigated the effect of adding well-known occlusion augmentation approaches such as Cutout \citep{devries2017cutout} and CutMix \citep{yun2019cutmix}. The results are shown in Table \ref{tab:occlusion}. Compared to the base counting network CSRNet+, both Cutout and CutMix reduce the counting error, but cannot compete with our occlusion simulation (Part\_A: 61.2~\citep{devries2017cutout}, 60.6~\citep{yun2019cutmix}, and 59.1 for ours - UCF\_QNRF: 91.8~\citep{devries2017cutout}, 90.6~\citep{yun2019cutmix}, and 87.4 for ours). Especially, our approach works much better when occlusion levels are high (Part\_A: 95.0~\citep{devries2017cutout}, 94.3~\citep{yun2019cutmix}, and 91.2 for ours - UCF\_QNRF: 104.7~\citep{devries2017cutout}, 103.1~\citep{yun2019cutmix}, and 99.3 for ours). This experiment solidifies our point: occlusions weight heavily on the counting error, and there are not enough natural occlusions to learn from. Instead, by simulating occlusions, we can easily reduce the MAE effectively.

%===============================
\subsection{Comparative evaluation} \label{exp}
%===============================
For the final experiments, we first show the effect of combining the four ways of focus we propose for improving transformation from input images to density maps by repurposing point annotations. Then we compare to the state-of-the-art in counting. 

\textbf{Combining the three focuses.} Until now, we have established that every solution plays a significant role in counting on its own. In this study, we aim to assess whether these solutions are also complementary to each other. The results of this experiment are shown in Table \ref{tab:combine}, utilizing both CSRNet+ and T2T-Vit as backbones. Our approach incorporates foreground focus using cascading segmentation and foreground distillation (detailed in section \ref{sec:segmentation}), which effectively reduces MAE when compared to standard counting with only the base networks. Moreover, by combining either global density focus (section \ref{sec:global}) or focus by simulating occlusion (section \ref{sec:occlusion}), we were able to further decrease the MAE. When we combine all three solutions, we observe the lowest count error across datasets and base networks.
%
\begin{figure*}[h!]
\centering
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/case/case_img.pdf}
\caption{\textbf{Input image}}
\label{fig:augmentation-a}    
\end{subfigure}
\begin{subfigure}{0.246\textwidth}
\includegraphics[width=\textwidth]{figures/case/case_seg.pdf}
\caption{\textbf{Cascade image}}
\label{fig:augmentation-b}    
\end{subfigure}
\begin{subfigure}{0.243\textwidth}
\includegraphics[width=\textwidth]{figures/case/case_density.pdf}
\caption{\textbf{Our density}}
\label{fig:augmentation-c}    
\end{subfigure}
\begin{subfigure}{0.243\textwidth}
\includegraphics[width=\textwidth]{figures/case/case_gt.pdf}
\caption{\textbf{Ground-truth}}
\label{fig:augmentation-d}    
\end{subfigure}
\caption{\textbf{Success and failure cases.} Illustrative examples of success and failure cases. When objects are individually visible, we can count them accurately (first three rows). Further improvements are required for extremely dense scenes where individual objects are hard to distinguish, or where objects blend with the context (last two rows). }
\label{fig:cases}    
\end{figure*}

\textbf{Comparison to the state-of-the-art.}
As the ultimate test, we draw a comparison to the state-of-the-art in counting on five datasets.
We report our results using both CSRNet+ and T2T-Vit as base networks, and both $ell_1$ and distribution matching (DM) \cite{wang2020distribution} as loss functions. Table \ref{tab:sota} shows the comparative evaluation over all datasets and metrics. The results show that despite using canonical counting backbones, which on their own can not compete with the state-of-the-art, we obtain the best density-based counting results on 8 of the 10 metrics. This highlights the potential of our simple solutions. We also compare to recent point-based counting alternatives and find that we maintain the best results for 6 of the 10 metrics. On ShanghaiTech Part\_A, we score below 50 in terms of MAE for the first time. We conclude that with our proposed solutions, we can make density-based optimization the most effective way to count again.
%
We show some success and failure results in Figure~\ref{fig:cases}. Even in challenging scenes with relatively sparse small objects or relatively dense large objects, our method is able to achieve an accurate count (first three rows). Our approach fails when dealing with extremely dense scenes where individual objects are hard to distinguish, or where objects blend with the context (last two rows). Such scenarios remain open counting challenges.

%\subsection{More analysis}
%\textbf{Complexity analysis.}
%The distilled density maps and occlusion simulations do not change inference time. Only the segmentation cascade adds complexity and increases the inference time, \eg, from 0.27s to 0.53s per image for the UCF\_QNRF dataset.
%\psmm{Do we have more analyses? Otherwise better to add this text to the implementation details.}
%The occlusion simulation relies on the size of objects. Currently, we use $2\sigma$ as an approximation to the size of an object. Since $\sigma$ is not estimated perfectly, a part of objects or the background is likely copied, which may affect the counting performance.

==> temp2.tex <==
\section{Method}
\label{sec:method}

%\cs{There is too much `focus-talk' in this section, if you call everything focus you may as well leave the word out. The information value becomes zero and irritates the reader.}

This work considers learning to count in a supervised manner, in which the training samples are provided as images and their corresponding point annotations. For density-based counting, the point annotations are generally used to generate Gaussian-density maps, which then serve as the supervision signal. This work starts from the premise that point annotations are a rich source of annotations with value for counting beyond generating density maps. We provide three ways to re-purpose the already available point annotations to improve counting. Below, we start by introducing how to formulate counting as a density map regression problem, and then outline the three ways to repurpose point annotations for improving counting, shown as an overview in Figure~\ref{fig:focus-overall}. First, we present a foreground distillation, which involves generating foreground masks from point annotations. This approach is effective in limiting the impact of background pixels on counting accuracy. Second, we introduce a counting-specific occlusion augmentation that utilizes point annotations on both input and density images to enhance the network's robustness to occlusions. Third, we introduce focus-for-free that generates both local and global focus for free with explicit supervision derived from point annotations.
%\cs{Need to explain the three methods briefly? Else the reader cannot follow the figure?}


\begin{figure*}[t!]
\centering
\includegraphics[width=0.9\linewidth]{figures/focus-overall.pdf}
\caption{\textbf{Overview of our approach.} 
Top: We enhance density regression by re-purposing the point annotations to develop a foreground focus with the aid of a segmentation loss $\mathcal{L}_s$ (Section \ref{sec:segmentation}) and a global density focus with the aid of a global density classification loss (Section \ref{sec:global}). Bottom: We create an auxiliary network that is trained on images with blacked-out background areas with the supervision of a Gaussian-density map, which is generated from the point annotations. Subsequently, we distill the foreground knowledge learned by the auxiliary network into the density prediction network. \psmm{Add section reference for bottom part description and choose more conventional colors. Most notably, the bright blue of "global density focus" does not fit with the other colors. I recommend choosing colors from a known color palette, see e.g. https://www.flerlagetwins.com/2021/06/datafam-colors-color-palette.html} \cs{Agree. This looks very clumsy. Certainly not IJCV-worthy.}
}
\label{fig:focus-overall}    
\end{figure*}

\subsection{Problem formulation}
We formulate the counting task as a density map regression problem, see \eg \cite{lempitsky2010learning,zhang2016single,Shi_2018_CVPR}. Density-based counting relies on point annotations indicating the locations of objects in training images. These annotations are typically represented as a set of coordinates $\mathcal{P}$, where each point $P{=}(x,y) \in \mathcal{P}$ corresponds to an object's location. From the point annotations we create a Gaussian-density map through convolutions with a normalized Gaussian kernel:
%
\begin{equation}
D(p)=\sum_{i=1}^N\mathcal{N}\big(p|\mu=P,\sigma_P^2\big),
\label{eq:density}
\end{equation}
%
where $p$ denotes a pixel location, and $\mathcal{N}(\cdot)$ is a normalized Gaussian kernel with mean $P$ and an isotropic variance $\sigma_P$. Determining $\sigma_P$ for each point $P$ is difficult because of object-size variations caused by perspective distortions. A solution is to estimate the radius $r$ of an object as a function of the $K$ nearest neighbor annotations, as done in the Geometry-Adaptive estimation of \cite{zhang2016single}. 

Our approach involves training a deep neural network $f$ to learn how to map images $I_i$ to their corresponding Gaussian-density maps $D_i$, forming a dataset ${(I_i,D_i)}_{i=1}^{N}$. To accomplish this, we optimize the parameters of $f$ using both the images and their associated density maps. During inference, we can obtain the global object count $T_i$ of an input image $I_i$ by summing all the pixel values within the predicted density map $\hat{D}i = f(I_i)$, as follows: $T_i = \sum{p \in I_i} \hat{D}_i(p)$. This operation integrates the predicted density values across the image domain and provides an estimate of the number of objects present in the image.

\subsection{Foreground distillation}
\label{sec:segmentation}
Typically, a network for density map prediction is learned by optimizing a loss function of the form
$\mathcal{L}_d{=} \ell_p(f_d(I)-D)$
where $f_d$ the network, $I$ the input image, $D$ the Gaussian-density map, and $\ell_p$ the Lp norm loss function. We can reformulate the loss function by dividing the density map into two components, one representing the background of the input image and the other corresponding to the foreground containing the objects of interest:
$\mathcal{L}_d{=} \ell_p({f_d(I)}_{bg}) + \ell_p({f_d(I)}_{fg}-D_{fg})$,
where $D_{bg}$ is naturally omitted as every single element in it is zero. Based on this reformulation, we identify two issues with current approaches. First, when $\ell_p({f_d(I)}_{bg})$ is not optimized perfectly, they are prone to misidentifying the background as objects (densities). Second, while trying to transform objects into densities, they cannot fully utilize their learning capacity as they predict densities by ${f_d(I)}_{fg}$ not only on objects but also on the background. 
To overcome these challenges, we propose a solution that ignores the background of the input image from the start. If we could remove all background pixels from the input image, ${f_d(I)}_{bg}$ would naturally be zero. Then the loss function becomes: $\mathcal{L}_d{=} \ell_p({f_d(\tilde{I})}_{fg}-D_{fg})$ with $\tilde{I}$ the image with zeros for background pixels. With this loss the network fits densities only on the objects.

\textbf{Focus from Foreground segmentation.} To reduce the impact of background pixels from the start, we propose a solution that re-purposes point annotations to create a binary segmentation map used to train a segmentation network capable of distinguishing between foreground and background areas. Specifically, we obtain a binary segmentation ground truth map $S$ as a function of the point annotations and their estimated variance. The binary value for each pixel location $p$ is determined as:
\begin{equation}
S(p) =
\begin{cases}
1 & \text{if  $\exists_{P \in \mathcal{P}} \big( ||p - P||^2 \leq \sigma_P^2$} \big),\\
0 & \text{otherwise.}
\end{cases}
\label{eq:segfocus}
\end{equation}
Equation~\ref{eq:segfocus} states that a pixel $p$ obtains a value of one if at least one point $P$ is within its variance range $\sigma_P$ as specified by a kernel estimator. By utilizing the obtained segmentation map as supervision, we train a segmentation network, $f_s$, which learns to distinguish between the foreground and background regions by optimizing a per-pixel weighted focal loss:
\begin{equation}
%\begin{split}
\mathcal{L}_s = 
 \sum_{{l} \in \{0,1\}} -\alpha{^l} S^l (1-\hat S)^{\gamma_s} log(\hat S),
\label{eq:focus-seg}
%\end{split}
\end{equation}
where $\alpha{^l}=1-\frac{|S^l|}{|S|}$ and $\hat S{=}f_s(I)$ the predicted segmentation map. The focal parameter $\gamma_s$ is set to 2 throughout this network, as recommended by \cite{lin2017focal}. 

We utilize the predicted segmentation map $f_s(I)$ to highlight the desired foreground areas while suppressing false background areas in the input image. The resulting loss function becomes
\begin{equation}
\mathcal{L}_d {=} \ell_p \Big(f_d\big(I\odot {f_s(I)}\big)-D\Big).
\end{equation}
With this approach, the network only fits densities on the objects, avoiding the impact of background pixels from the start.

\textbf{Foreground distillation.} Achieving a perfect foreground segmentation is a challenging task and any imperfections may reduce the effectiveness of the foreground focus. We propose a solution to this issue by learning how to distill true foreground knowledge. In particular, we have developed an auxiliary network that we train on images where background areas are blacked-out. The training loss is
\begin{equation}
\label{eq:auxiliary}
  \mathcal{L}_a{=} \ell_p \big({f_a(I\odot S)}-D\big),
\end{equation}
where $f_a$ is the auxiliary network, $I\odot S$ the image with background areas blacked-out, $S$ the segmentation ground truth, and $D$ the Gaussian-density map. The optimization of the auxiliary network will be stopped when it achieves maximum accuracy on the validation set. Then we distill the knowledge of the trained auxiliary network to the density prediction network with the loss
\begin{equation}
\label{eq:distillation}
  \mathcal{L}_d{=} \ell_p \big(\hat{D} - f_a(I\odot S)\big),
\end{equation}
where $\hat{D}$ represents the density map predicted with our foreground focus, which can be obtained by $f_d(I)\odot f_s(I)$ or $f_d\big(I \odot f_s(I)\big)$. Unlike traditional distillation methods that aim to compress information \citep{hinton2015distilling}, our distillation technique aims to extract foreground knowledge. In the density prediction loss function $\mathcal{L}_d$, we replace the Gaussian density map with our distilled density map for the final training, rather than do both. Foreground knowledge distillation is only performed during the training phase, hence it does not impact inference time.
%Our distillation loss is not combined with the ground truth loss because we observed that combining the two leads to a reduction in counting performance. \psmm{Previous sentence unclear, do you mean that we replace the Gaussian density map with our distilled density map for the final training, rather than do both?} 

\subsection{Global density focus}
\label{sec:global}
Aside from providing a spatial focus through foreground segmentation, point annotations can also be re-purposed to achieve a channel focus by examining contextual information through global density classification. In dense prediction tasks, it is crucial to comprehend and leverage contextual information. In the context of per-pixel density prediction for counting, global context is associated with the overall crowd density in the image. To capture such global context, we learn a global density classification task. We then utilize this captured global context to develop a channel focus that highlights feature maps that align with the global density reflected by the annotation points, leading to improved counting performance.

\textbf{Global density classification.} To perform global density classification, we first obtain a global density ground truth from the point annotation, for free. Specifically, the global density for a patch $j$ in the training image $i$ is given as:
\begin{equation}
G_{j,i} = \frac{|\mathcal{P}_{j,i}|}{L}, L = \left \lfloor{ \max_{i=1,..,N} \Big (\frac{|\mathcal{P}_{i}|}{Z_i} \cdot Z_{j,i}\Big) / M}\right \rfloor + 1.
\end{equation}
Here $|\mathcal{P}_{j,i}|$ denotes the number of object points in patch $j$, $L$ denotes the global density step size, $Z_i$ and $Z_{j,i}$ denote the number of pixels in image $i$ and patch $j$ respectively. The step size calculation involves determining the highest global density across image patches, while the parameter $M$ denotes the number of global density levels used in the process. By leveraging the global density ground truth, we train a network $f_c$ for classifying global density with the following loss:
\begin{equation}
\mathcal{L}_c = 
\sum_{{l} \in \{0,1,..,M\}} -G^l (1-\hat G)^{\gamma_c} log(\hat G),
\label{eq:global density}
\end{equation}
where $\hat G{=}f_c(I)$ and $\gamma_c$ is set to 2. The $f_c$ model comprises a backbone network and a classifier. The backbone network is shared with the per-pixel density prediction network $f_d$. To capture feature statistics in a global context, we incorporate a global average pooling on top of the backbone network. The classifier comprises two fully-connected layers and a softmax function. 

%\textbf{Focus from global density classification.} 
After capturing the global context, we develop a channel focus that emphasizes feature maps aligned with the global density. To achieve this, we employ two fully-connected layers followed by a sigmoid function on top of the bilinear pooling layer, which generates a global density focus output. The resulting focus output is then utilized by the density prediction network's backbone to highlight feature maps that exhibit similar global contextual patterns to the ground truth density maps. %This leads to enhanced counting results.
%\psmm{explain here how global context is embedded in overall framework, i.e. how is it linked with the density estimation?}

\begin{figure}[t!]
\centering
\includegraphics[width=\columnwidth]{figures/global_density.pdf}
\caption{\textbf{Global density focus.} Bilinear pooling extracts essential global context information. Then two distinct branches process the resulting context. The top branch, consisting of an MLP and a sigmoid function, generates a focus map that highlights important feature maps. The bottom branch, comprising an MLP and a Softmax function, enhances the extracted context by learning to classify global density. \psmm{Match colors with updated Figure 1}}
\label{fig:segmentation}    
\end{figure}


\begin{figure}[t!]
\centering
\begin{subfigure}{\linewidth}
\includegraphics[width=\textwidth]{figures/occlusion_density.pdf}
\caption{\textbf{Occlusion simulation for point annotations}}
\label{fig:augmentation-a}    
\end{subfigure}
\begin{subfigure}{\linewidth}
\includegraphics[width=\textwidth]{figures/occlusion_image.pdf}
\caption{\textbf{Occlusion simulation for image}}
\label{fig:augmentation-b}    
\end{subfigure}
\caption{\textbf{Occlusion simulation.} (a): We randomly choose two object points from an object point map, one for the object which will be occluded, denoted by $\mathcal{O}_{occ}$ and another for the object which will be copied and pasted, denoted by $\mathcal{O}_{copy}$. The pasted position of $\mathcal{O}_{copy}$ is computed based on Eq. (\ref{eq:occlusion}), as indicated by $\mathcal{O}_{paste}$.
%
(b): We generate an occluded image  from $\mathcal{O}_{occ}$, $\mathcal{O}_{copy}$, and $\mathcal{O}_{paste}$. To avoid boundary artifacts, we perform blending to smooth out the boundary artifacts. \psmm{Match colors with updated Figure 1}
}
\label{fig:cases}    
\end{figure}


\subsection{Focus by simulating occlusion}
\label{sec:occlusion}
Finally, we utilize annotation points to augment overlapping objects to overcome the occlusion challenge. Occlusions often happen in congested scenes, resulting in overlapping objects. For counting purposes, one  solution to handle various occlusion levels is to learn a network with sufficient number of training samples for each occlusion level. However, the occlusion level presents a long-tailed distribution in all benchmarks  \citep{zhang2016single,idrees2018composition,sindagi2020jhu-crowd++,guerrero2015extremely}. In other words, there are simply not enough images in current datasets to properly learn from natural occlusions. As a remedy, we propose to simulate various occlusion levels through augmentation.

\textbf{Occlusion simulation.} 
Given a training sample consisting of an input image and its point annotations, $(I, {P_i}{i=1}^{N})$, we represent any object $\mathcal{O}_i$ in the image $I$ as $(x_i,y_i,2\sigma_i)$. Here, $(x_i, y_i)$ represents the coordinate of the corresponding annotated point $P_i$, and $\sigma_i$ is the variance of the corresponding Gaussian kernel. This representation assumes that the object $\mathcal{O}_i$ is circular and its radius is approximately equal to $2\sigma_i$, as proposed in~\cite{lempitsky2010learning}. To generate occlusion scenarios, we randomly select an object, $\mathcal{O}{occ}$, to be occluded. We then select one of its neighboring objects, denoted as $\mathcal{O}{copy}$, which will be copied and pasted to occlude $\mathcal{O}{occ}$. The pasted position of $\mathcal{O}{copy}$ determines how $\mathcal{O}_{occ}$ will be occluded, defined as: 
%
\begin{equation}
  \begin{aligned}
  x_{paste} &= \lfloor r \cdot cos(\theta) \rfloor + x_{occ},\\
  y_{paste} &= \lfloor r \cdot sin(\theta) \rfloor + y_{occ},
  \end{aligned}
  \label{eq:occlusion}
\end{equation}
%
where $r{=}r_{copy}+r_{occ} \epsilon_r$ and $\theta {=} 2\pi \epsilon_{\theta}$. $\epsilon_r$ and $\epsilon_{\theta}$ are randomly sampled from $\mathcal{U}(0,1)$. $\lfloor \cdot \rfloor$ is the floor operator. $r$ and $\theta$ decide how much and where $\mathcal{O}_{occ}$ will be occluded. 

\textbf{Blending.} Directly pasting objects on an image creates boundary artifacts, which may affect the network's learning ability. To handle boundary artifacts, we perform blending to smooth out the boundary artifacts. Specifically, we first copy and paste the object $\mathcal{O}_{copy}$ to the position $(x_{paste},y_{paste})$ of the image $I$, generating a new image $\hat I$. Then, we compute the binary mask $\alpha$ of the pasted object $\mathcal{O}_{paste}$, which we represent by $(x_{paste},y_{paste},r_{paste})$ where $r_{paste}{=}r_{copy}$. To smooth out the edges of the pasted object, we apply a Gaussian filter to the binary mask $\alpha$ and obtain a smoothed mask $\tilde \alpha$. From $\tilde \alpha$ we construct the occluded image $I_{occ}$ and its corresponding ground truth density map:
%
\begin{equation}
  \begin{aligned}
  I_{occ} &= (1-\tilde \alpha)\odot I + \tilde \alpha \odot \hat I,\\
  D_{occ} &= D + G(\mathcal{O}_{paste}),
  \end{aligned}
  \label{eq:blending}
\end{equation}
%
where $D$ denotes the ground truth density map of the image $I$, $G(\mathcal{O}_{paste})$ denotes the density map of the pasted object $\mathcal{O}_{paste}$, and $G$ denotes the Gaussian kernel. Equation \ref{eq:blending} states that the pixels to be occluded in the original image are replaced by the pixels of the pasted object to obtain the occluded image. The corresponding occluded density map is obtained by simply adding the density map of the pasted object to the original density map. 

\textbf{Occluding adaptively.} For a training image, we need to decide how many of its objects will be occluded with our approach. A simple way is to set a fixed ratio. However, the training image may already have naturally occluded objects. Thus, we should create new occlusion for the training image according to its current occlusion level. Intuitively, the lower the occlusion level, the higher the amount of occlusions that should be simulated. To compute the occlusion level, we create an occlusion map $M$ for the training image by,
% 
\begin{equation}
\begin{aligned}
&M(x,y) = \sum_{i=1}^N S(x,y;\mathcal{O}_i), \text{where} \\ &S(x,y;\mathcal{O}_i) = \mathds{1}(||x - x_i||^2 + ||y - y_i||^2 \leq (r_{i})^2). 
\end{aligned} 
\label{eq:occmap} 
\end{equation}
%
Here $(x,y)$ denotes a pixel location, $\mathcal{O}_i{=}(x_i,y_i,r_{i})$ denotes an object, and $\mathds{1}(\cdot)$ is a binary indicator function, which states that a pixel obtains a value of one if it is within an object region. Hence, each pixel value in the occlusion map $M$ indicates the amount of object regions it belongs to. The occlusion level $\bar M$ is computed as the average value of non-zero pixels in the occlusion map $M$. Then the percentage of the objects to be occluded can be adaptively obtained by $\beta $/$\bar M$ where $\beta$ is the upper boundary, and $\beta{=}0.3$ empirically performs well.

\subsection{Transformer with focus-for-free}
\label{sec:transformer}

\cs{Need to discuss structure of section 3, I get a bit confused by all the bells and whistles that are introduced and how they are related. I did not see this transformer in Figure 1. How related? Also, what is new? Isn't it just implementation details?}

Transformer architectures have shown significant promise in  counting and is quickly becoming the preferred backbone. As a result, we are inspired to incorporate our foreground focus and global density focus in transformers and leverage their capabilities to further advances counting models.

\textbf{Token-to-token Encoder.} Instead of relying on the basic tokenization approach employed in Vit \citep{dosovitskiy2020image}, we adopt the progressive tokenization module introduced by \cite{yuan2021tokens}. This module enables us to aggregate adjacent tokens into a single token, thereby incorporating local structural information from surrounding tokens and reducing the token length in a step-by-step manner. To be more specific, we utilize a Token-to-Token (T2T) mechanism, where tokens produced by a transformer layer are first reconstructed as an image, then split into overlapping patches, and finally aggregated by flattening the patches. This process allows the local structure of surrounding patches to be embedded into the tokens, which are subsequently fed into the next transformer layer. By performing T2T iteratively, the local structure is integrated into the tokens, and the token length is reduced via the aggregation process. Finally, we use an efficient deep-narrow backbone structure for the vision transformer to learn the representations from these tokens. 

\textbf{Foreground focus decoder.} To design the decoder for foreground focus, we have adopted a multi-level feature aggregation approach inspired by the feature pyramid network \cite{kirillov2019panoptic}. However, instead of using a pyramid shape, we leverage the feature representations from different layers of the T2T-Vit encoder, which have the same resolution. We begin by selecting $m$ layers from the encoder, uniformly distributed across the layers with a step of $n$. We then deploy $m$ streams, each focusing on one specific selected layer. In each stream, we first reshape the encoder's feature $Z^l$ from a 2D shape to a 3D feature map. Next, we apply a 3-layer convolutional network to process the feature from each stream. To promote interactions across different streams, we introduce a top-down aggregation design through element-wise addition after the first layer. An additional $3\times3$ convolution layer is applied after the element-wise auditioned feature. After the third layer, we obtain the fused feature from all the streams via channel-wise concatenation. This feature is then upsampled $2\times$ to match the resolution of the output density map.

\textbf{Global density focus decoder.} To capture global context information and improve it using a global density classification loss, we employ a bilinear pooling when CNN is used as encoder. However, when using a vision transformer as the encoder, we assign the task of capturing global context to a global density class token.
we use the global density class token to predict global density. To achieve this, two fully-connected layers with Softmax activation is utilized. Additionally, this token serves as the primary input to the global density focus module, which consists of two fully-connected layers with a Sigmoid activation. The global density focus module's objective is to refine the local feature map used for crowd density map prediction, given the global density class token. By doing so, the network can focus on critical feature channels, resulting in improved features.

\psmm{Maybe a figure with the overall new transformer architecture is helpful? to discuss}

==> temp3.tex <==
\section{Experiments and results}
We first describe the experimental setup. We then analyze the effect of three methods of repurposing point annotations proposed in this work, comparing each to their respective baseline approaches. Finally, we report the results of the combination of the three methods and compare them to the state-of-the-art.
%===============================
\subsection{Experimental setup}
%===============================
\textbf{Datsets.}  We consider five counting datasets in this paper commonly used in the recent literature, \eg,~\citep{bai2020adaptive,wan2021generalized,liu2021exploiting,wang2021uniformity,song2021rethinking,ma2021towards}:
%
\textbf{\textit{ShanghaiTech}} \citep{zhang2016single} consists of 1,198 images with 330,165 pedestrians. This dataset is divided into two parts: \textbf{\textit{Part\_A}} with 482 images in which crowds are mostly dense, and \textbf{\textit{Part\_B}} with 716 images, where crowds are sparser. Each part is divided into a training and testing subset as specified in \citep{zhang2016single}. 
%
\textbf{\textit{UCF-QNRF}} \citep{idrees2018composition} consists of 1,535 images, with the count ranging from 49 to 12,865. 
For training 1,201 images are available, and the remaining 334 form the test set. 
%
\textbf{\textit{JHU-CROWD++}} \citep{sindagi2020jhu-crowd++} consists of 4,372 images with a total of 1.51 million point annotations. 
The dataset is split into a training set of 2,272 images, a validation set of 500 images and a testing set of 1,600 images.
\textbf{\textit{NWPU-Crowd}} \citep{wang2020nwpu} consists of 5,109 images with over 2 million point annotations. 
The dataset is split into a training set of 3,109 images, a validation set of 500 images and a testing set of 1,500 images. 

For all datasets, we augment the images by randomly performing horizontal flipping, and randomly cropping $256 {\times} 256$ patches for ShanghaiTech, JHU-CROWD++ and $416 {\times} 416$ patches for UCF-QNRF, NWPU. For Gaussian density map generation, we follow the previously suggested dataset settings from \citep{zhang2016single,idrees2018composition,sindagi2020jhu-crowd++}.

\textbf{Implementation details.} 
We adopted T2T-ViT-14 \citep{yuan2021tokens} as our transformer backbone network and integrated our methods using the guidelines outlined in section \ref{sec:network}. Additionally, we incorporated CSRNet \citep{Li_2018_CVPR} as our convolutional backbone network. CSRNet has been widely used in the literature, as demonstrated by its inclusion in multiple studies \citep{zhao2019leveraging,ma2019bayesian,wan2020modeling,wang2020distribution,wan2021generalized,ma2021towards}. To enhance its performance, we introduced batch normalization layers into our implementation of CSRNet, similar to the approach taken by \cite{bai2020adaptive}. This improved version is called CSRNet+. For our integration with CSRNet+, we used the same backbone network as the frontend network and the same focus from segmentation module and density regressor module as the backend network. The focus from the global density module is the same as that used with T2T-ViT-14, but we employed a bilinear pooling layer instead of using the global density class token. Both networks have been initialized with their ImageNet pre-trained models and trained using Adam with batches of 10. By default, we have used an $\ell_1$ loss function. The learning rate has been fixed at 1e-4 for CSRNet+ and le-5 for T2T-ViT-14.

\textbf{Metrics.} We report the standardized Mean Absolute Error (MAE) and Root Mean Square Error (RMSE) metrics given count estimates and their ground-truth.
%
\begin{table}[!t]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{@{}lcccccccccccccccc@{}}
\toprule
& \multicolumn{2}{c}{\textbf{CSRNet+}} &
\multicolumn{2}{c}{\textbf{T2T-Vit}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& \textit{Part\_A} & \textit{UCF\_QNRF} & \textit{Part\_A} & \textit{UCF\_QNRF}\\
\hline
Standard  &61.9 &93.6 & 60.1 &90.8\\
w/o background &29.8 &57.4 &27.7 &54.6\\
\bottomrule
\end{tabular}}
\caption{\textbf{Impact of background error.} Removing the background pixels with an oracle before density prediction reduces the count error (MAE) considerably across datasets and networks.}
\label{tab:seg}
\end{table}
%
%
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{}lccccccccccccccc@{}}
\toprule
& \multicolumn{6}{c}{\textbf{\textbf{CSRNet+}}} & \multicolumn{6}{c}{\textbf{\textbf{T2T-Vit}}}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} & \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
& \textit{BG}  & \textit{FG}  & \textit{Overall} & \textit{BG} & \textit{FG} & \textit{Overall} & \textit{BG}  & \textit{FG}  & \textit{Overall} & \textit{BG} & \textit{FG} & \textit{Overall} \\
\hline
Base network & 3.4 & 61.5 & 61.9 &8.7 & 91.3 &93.6 & 3.2 & 59.1 & 60.1 &8.2 & 89.7 &90.8\\
w/ attention-injective \citep{liu2019adcrowdnet} & 3.3 & 59.7 & 60.5 &6.1 & 89.9 &91.2 & 3.0 & 58.5 &59.1 &5.8 & 89.1 &89.8\\
w/ focus from segmentation\citep{shi2019counting} & 3.2 & 59.1 & 59.6 &5.2 & 89.6 &90.3 & 3.1 & 58.2 &58.5 &4.9 & 89.4 &89.1 \\
w/ segmentation attention \citep{modolo2021understanding} & \textbf{2.9} & 58.8 & 59.3 &4.5 & 88.3 &89.4 & \textbf{2.8} & 57.7 &58.2 &4.4 & 88.3 &88.8 \\
w/ background feature filtering \citep{mo2020background} & 3.1 & 58.2 & 58.8 &4.3 & 87.1 &88.3 &2.9 & 57.1 &57.7 &4.8 & 87.6 &87.9 \\
w/ decoupled learning \citep{cheng2021decoupled} & 3.1 & 57.1 & 57.5 &3.5 &84.8 &85.6 &3.0 & 55.6 &56.4 &\textbf{4.2} & 83.8 &84.4\\
\hline
\rowcolor{Gray}
w/ our input-foreground focus & 3.0 & \textbf{55.3}&\textbf{56.1}&\textbf{3.4}& \textbf{83.6} &\textbf{84.4} &2.9& \textbf{54.2} &\textbf{55.4} &4.8 &\textbf{82.7} &\textbf{83.6}\\
\bottomrule
\end{tabular}
\end{threeparttable}}
\caption{\textbf{Effect of foreground focus.} Compared to base networks and our reimplementation of four related works, which predict density maps on the background, our simple cascade model with background reduction reduces the overall count error (MAE), for both background (BG) and foreground (FG).  
}
\label{tab:seg+dis}
\end{table*}
%
%
\begin{figure*}[t!]
\centering
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/cascade/cascade_input.pdf}
\caption{\textbf{Input image}}
\label{fig:segmentation-a}    
\end{subfigure}
\begin{subfigure}{0.245\textwidth}
\includegraphics[width=\textwidth]{figures/cascade/cascade_seg.pdf}
\caption{\textbf{Cascaded image}}
\label{fig:segmentation-b}    
\end{subfigure}
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/cascade/cascade_density.pdf}
\caption{\textbf{Our density}}
\label{fig:segmentation-c}    
\end{subfigure}
\begin{subfigure}{0.243\textwidth}
\includegraphics[width=\textwidth]{figures/cascade/cascade_gt.pdf}
\caption{\textbf{Ground-truth}}
\label{fig:segmentation-d}    
\end{subfigure}
\caption{\textbf{Learning to avoid the background.}  Segmentation and density prediction results by our cascade model. While by no means perfect, the predicted segmentation masks already reduce the background pixels considerably. The density prediction network is then able to count correctly on the remaining amount of background pixels, as masked in the green regions. }
\label{fig:segmentation}    
\end{figure*}
%===============================
\subsection{Foreground focus}
\label{sec:exp_segmentation}
%===============================
\textbf{Impact of background interference.}
In section \ref{sec:segmentation}, we introduce the input-foreground focus techniques that aim to reduce the impact of background interference in input images. Before evaluating the effectiveness of this method, we need to quantify how much the background impedes counting performance. To accomplish this, we use oracle segmentation maps based on Eq. \ref{eq:segfocus}. To examine the background error, we use the oracle segmentation map to mask the input image itself and then apply the baseline counting network to the masked image to predict the density map. It's worth noting that the original input image and its background-free equivalent share the same ground-truth density map.

Table~\ref{tab:seg} presents the results of our experiments on two counting networks and two datasets. The results consistently show that by predicting the density maps without the background, the counting error can be significantly reduced. For instance, on the ShanghaiTech Part\_A dataset, CSRNet+ reduces the MAE from 61.9 to  29.8 by predicting the density maps without the background. This result surpasses the current state-of-the-art on this dataset by a considerable margin. Our findings suggest that the interference caused by the input image's background could be responsible for most of the counting error. In conclusion, our oracle experiment highlights that removing the background from the input image can significantly enhance density-based counting.

\textbf{Effect of focus from foreground segmentation.}
Motivated by the oracle experiment, our counting model with input-foreground focus cascades a segmentation network and a density prediction network to reduce the impact of background pixels from the start. To emphasize that the key is to remove the background from the input image altogether, we compare it to the other five baselines. The first baseline \cite{liu2019adcrowdnet} is a cascade counting approach, which cascades a crowd-level attention prediction network and a density estimation network. The second baseline is our previous focus from segmentation \citep{shi2019counting}. The third baseline \citep{modolo2021understanding} reduce the background error by learning a segmentation attention map for the output density map. The fourth one \citep{mo2020background} filters the background noise on the intermediate features by learning a head segmentation mask.
%
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{cccccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Foreground focus}} & \multicolumn{2}{c}{\textbf{CSRNet+}}&\multicolumn{2}{c}{\textbf{T2T-Vit}} \\
\cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}
Foreground distillation & Input-foreground focus  &\textbf{Part\_A} & \textbf{UCF\_QNRF} &\textbf{Part\_A} & \textbf{UCF\_QNRF}  \\
\hline
 & & 61.9 & 93.6&60.1 &90.8 \\
\rowcolor{Gray}
 \checkmark& &56.7&87.9&- &-\\
  &\checkmark&56.1&84.4&55.4&83.6\\
\rowcolor{Gray}
 \checkmark&\checkmark  &\textbf{54.6}&\textbf{81.7}&\textbf{-}&\textbf{-}\\

\bottomrule
\end{tabular}
\end{threeparttable}}
\caption{\textbf{Effect of foreground distillation.} Foreground distillation significantly improves the performance when used directly with the base network, or in conjunction with output-foreground focus or in-foreground focus.}
\label{tab:seg+dis}
\end{table*}
%
%
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{}lccccccccccccccc@{}}
\toprule
& \multicolumn{6}{c}{\textbf{\textbf{CSRNet+}}} & \multicolumn{6}{c}{\textbf{\textbf{T2T-Vit}}}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} & \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
& \textit{sparse}  & \textit{dense}  & \textit{Overall} & \textit{sparse}  & \textit{dense}  & \textit{Overall} & \textit{sparse}  & \textit{dense}  & \textit{Overall} & \textit{sparse}  & \textit{dense}  & \textit{Overall} \\
\hline
Base network & 35.8 & 88.0 &61.9 &50.8 & 136.4 &93.6 &37.4 &82.8 &60.1 &- &- &-\\
w/ CBAM \citep{woo2018cbam} &36.5 &85.9 &61.2 &51.7 & 131.9 &91.8 &36.8 &82.6 &59.7 &- &- &-\\
w/ SE \citep{hu2018squeeze} & 36.9 &84.3 & 60.6 &51.3 & 129.7 &90.5 &36.1 &82.7 &59.4 &- &- &-\\
\rowcolor{Gray}
w/ our global density focus& 35.0 & 83.2 & 59.1 &50.2 & 127.0 &88.6 &35.5 &81.9 &58.7 &- &- &-\\
\bottomrule
\end{tabular}
\end{threeparttable}}
\caption{\textbf{Effect of global density focus.} Our approach, which incorporates explicit supervision for channel attention, outperforms both the base networks and two related works that implement channel attention implicitly. Our method significantly reduces the mean absolute error (MAE) for both sparse and dense crowd counting. 
}
\label{tab:gf}
\end{table*}
%
The last baseline \cite{cheng2021decoupled} learns to count with decoupled learning, which first regresses a probability map to identify possible object regions, and then predicts a density map on the probability map to count the objects. As shown in Table~\ref{tab:seg+dis}, all five baselines perform better than the base network only, while our method even better improves both background and foreground errors, with a special focus on the foreground error. With the CSRNet+ base network, for instance,  on ShanghaiTech Part\_A our approach provides a reduction of 5.8 in the overall MAE. On UCF \_QNRF, the overall MAE even goes down by 9.2. The results emphasize the importance of removing the background in the input image for counting. We also provide qualitative results in Figure \ref{fig:segmentation}. We observe that our predicted segmentation masks remove many background pixels, and the density prediction network is able to count well on the remaining pixels. 
%
Overall, we recommend learning to remove the background from the input image for density-based counting. The gap towards oracle performance further highlight that big gains should be feasible with more advanced image segmentation.

\textbf{Effect of foreground distillation.}
We have conducted experiments to evaluate the effectiveness of our proposed foreground distillation when used directly with the base network, or in conjunction with in-foreground focus. Our results, shown in Table~\ref{tab:seg+dis}, indicate that foreground distillation significantly improves the performance in all two scenarios. For example, using the base network CSRNet+ alone, our approach reduces MAE by 3.2 on ShanghaiTech Part\_A. With the addition of input-foreground focus, the MAE further goes down by 5.8, respectively. Foreground distillation is a simple yet effective approach that can be easily applied to any network, resulting in a direct reduction in counting errors. 
%
\begin{table*}[!t]
\renewcommand{\arraystretch}{1.2}
\centering
\resizebox{0.99\linewidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{}lccccccccccccccc@{}}
\toprule
& \multicolumn{6}{c}{\textbf{\textbf{CSRNet+}}} & \multicolumn{6}{c}{\textbf{\textbf{T2T-Vit}}}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
& \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} & \multicolumn{3}{c}{\textbf{Part\_A}} &
\multicolumn{3}{c}{\textbf{UCF\_QNRF}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} 
& \textit{Low}  & \textit{High} &\textit{Overall}  & \textit{Low}  & \textit{High} & \textit{Overall}& \textit{Low}  & \textit{Dense} &\textit{High}  & \textit{Low}  & \textit{Dense} & \textit{High} \\
\hline
Base network & 39.2 & 95.9 & 61.9 &18.7& 106.5 &93.6 & 36.6 & 94.7 & 60.1 &17.8& 103.5 &90.8\\
w/ cutout \citep{devries2017cutout} & 38.6 & 95.0 & 61.2 &\textbf{16.5}& 104.7 &91.8 & 35.9 & 93.6 & 58.9 &\textbf{15.7}&101.9 &88.8\\
w/ cutmix \citep{yun2019cutmix} &38.0 & 94.3 &60.6 &17.8&103.1 &90.6 & 35.7 & 93.2 & 58.6 &16.4&99.6&87.5\\
\rowcolor{Gray}
w/ ours  &\textbf{37.8} & \textbf{91.2} &\textbf{59.1} &18.3& \textbf{99.3} &\textbf{87.4} &\textbf{34.9} & \textbf{90.7} & \textbf{57.2} &16.8& \textbf{98.3} &\textbf{86.3}\\
\bottomrule
\end{tabular}
\end{threeparttable}}
\caption{\textbf{Effect of our solution for occlusion error.} Compared to a base network and our reimplementation of two related works, our occlusion augmentation reduces the count error (MAE) for the entire test set, the \emph{low} occlusion set, and especially for the \emph{high} occlusion set. 
}
\label{tab:occlusion}
\end{table*}
%
%
\begin{figure*}[!t]
\centering
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/occ/img_ori.pdf}
\caption{\textbf{Original image}}
\label{fig:augmentation-a}    
\end{subfigure}
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/occ/img_ours.pdf}
\caption{\textbf{Our image}}
\label{fig:augmentation-b}    
\end{subfigure}
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/occ/den_ori.pdf}
\caption{\textbf{Original density}}
\label{fig:augmentation-c}    
\end{subfigure}
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/occ/den_ours.pdf}
\caption{\textbf{Our density}}
\label{fig:augmentation-d}    
\end{subfigure}
\caption{\textbf{Occlusion creation}. Illustrative examples for creating new occlusions on images and corresponding density maps. Our occlusion-augmented image and density look quite natural, as masked in the green regions.}
\label{fig:augmentation}   
\end{figure*}
%===============================
\subsection{Global density focus}
%===============================
Next, we demonstrate the effect of our proposed global density focus module. We compare it with the SE module \citep{hu2018squeeze} and the channel attention module of CBAM \citep{woo2018cbam}, while keeping the base network unchanged. To ensure a fair comparison, we use the same MLP network for all the approaches.

To evaluate the performance of our module, we define the crowding level of each image as $I_{crowd} = \frac{N(\mathcal{O})}{S(I)}$, where $N(\mathcal{O})$ represents the number of objects in the image, and $S(I)$ denotes the size of the image. We then sort the test images in ascending order based on their global density level and divide them uniformly into three sets: sparse, medium, and dense. By doing so, we demonstrate that our module exhibits a lower error on different crowding levels.

The results of our experiment are presented in Table \ref{tab:gf}. Both SE and CBAM can already improve the base network's performance based on both CSRNet+ and T2T-Vit. Our proposed global density focus outperforms SE and CBAM, reducing the count error even further, due to its explicit supervision. 
%
\begin{table*}[!t]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
\multicolumn{3}{c}{\textbf{Three ways of focus by repurposing point annotations}} & \multicolumn{2}{c}{\textbf{CSRNet+}}&\multicolumn{2}{c}{\textbf{T2T-Vit}} \\
\cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Foreground focus & Global density focus & focus by simulation &\textbf{Part\_A} & \textbf{UCF\_QNRF} &\textbf{Part\_A} & \textbf{UCF\_QNRF}  \\
\hline
 & & & 61.9 & 93.6&59.7 &90.4 \\
 \checkmark & & & 56.1&84.4&55.4 &83.6\\
 \checkmark&\checkmark &  &54.7 &82.2&53.4 &81.5\\
\checkmark& & \checkmark & 53.5 &81.2&51.2 &79.6\\
\rowcolor{Gray}
\checkmark&\checkmark & \checkmark & \textbf{52.4} & \textbf{79.8}& \textbf{49.1} & \textbf{78.2}\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Effect of combining our three focus solution} in terms of MAE on ShanghaiTech Part\_A and UCF\_QNRF. With each new addition, the counting error decreases, showing their complementary nature.}
\label{tab:combine}
\end{table*}
%
\begin{table*}[t!]
\centering
\resizebox{0.99 \linewidth}{!}{
\begin{tabular}{@{}lccccccccccccr@{}}
\toprule
&\multirow{2}{*}{\textbf{Backbone}} &\multicolumn{2}{c}{\textbf{Part\_A}} & \multicolumn{2}{c}{\textbf{Part\_B}}&\multicolumn{2}{c}{\textbf{UCF\_QNRF}}&\multicolumn{2}{c}{\textbf{JHU-CROWD++}}&\multicolumn{2}{c}{\textbf{NWPU-Crowd}}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}  \cmidrule(lr){11-12}
 & & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE & RMSE & MAE &  RMSE\\
\hline
\rowcolor{Gray} 
\textbf{Lp loss}&&&&&&&&&&&&\\
\cite{xu2022autoscale} &VGG-16&65.8 &112.1 &8.6 &13.9 &104.4 &174.2 &76.4&292.7&94.1&388.2\\
%
\cite{wan2020kernel} &VGG-16&63.8 &99.2 &7.8 &12.7 &99.5 &173.0 &69.7&268.3&100.5&415.5\\
% 
\cite{ma2021towards} &VGG-16&58.4 &97.9 &- &- &96.3&155.7 &65.1&269.3 &- &-\\
\cite{shu2022crowd} &VGG19&57.5&94.3 &6.9 &11.0 &80.3 &137.6 &57.0 &235.7 &76.8 &343.0 \\
%
\cite{cheng2021decoupled} &VGG-16&57.2 &93.0 &6.3 &10.7 &81.7&137.9 &73.7&292.5 &85.5 &361.5\\
%
\cite{bai2020adaptive} &VGG-16&55.4 &97.7 &6.4 &11.3 &\underline{\textbf{71.3}}&&- &- &- &-\\
%
\cite{tran2022improving} &ViT-B/32&54.8 &80.9 &8.6 &13.8 &87.0&141.9 &-&- &- &-\\
%
\cite{cheng2022rethinking} &ResNet-50&54.8 &89.1 &6.2 &9.9 &81.6&153.7 &58.2&245.1 &- &-\\
%
\cite{wang2021uniformity} &VGG-16&54.6 &91.2 &6.4 &10.9 &81.1&131.7 &-&- &- &-\\
%
\textit{\textbf{Ours (CSRNet+)}} &VGG-16&- &- &- &- &-&- &-&- &- &-\\
%
\textit{\textbf{Ours (T2T-Vit)}} &T2T-Vit-14&\underline{\textbf{49.1}} &\underline{\textbf{83.2}} &\underline{\textbf{6.1}} &10.3 &78.2& \textbf{126.5} &\underline{\textbf{56.8}}&253.4 &\underline{\textbf{-}} &\underline{\textbf{-}}\\
%
\midrule
\rowcolor{Gray} 
\textbf{DM loss}&&&&&&&&&&&&\\
%
\cite{wan2021generalized} &VGG19&61.3 &95.4 &7.3 &11.7 &84.3&147.5 &59.9&259.5 &79.3 &346.1\\
%
\cite{wang2020distribution}  &VGG-19&59.7 &95.7 &7.4 &11.8 &85.6 &148.3 &- &- &88.4 &388.6 \\
%
\cite{liu2021exploiting} &ResNet-18&55.4 &91.3 &6.9 &10.3 &76.2&\underline{121.5} &59.9&259.5 &\underline{74.7} &\underline{267.9}\\
%
\cite{ma2021towards} &VGG-19&55.0 &92.7 &- &- &80.7&146.3 &59.3&\underline{\textbf{248.9}} &- &-\\
%
\cite{sun2021boosting} &T2T-Vit-14&53.1 &82.2 &7.3 &11.5 &83.8&143.4 &54.8&208.5 &82.0 &366.9\\
%
\cite{song2021rethinking} &VGG-16&52.7 &85.1 &6.3 &\underline{9.9} &85.3&154.5 &-&- &77.4 &362.0\\
%
\textit{\textbf{Ours (CSRNet+)}} &VGG16&- &- &- &- &-&- &-&- &- &-\\
%
\textit{\textbf{Ours (T2T-Vit)}} &T2T-Vit-14&\underline{\textbf{-}} &\underline{\textbf{-}} &\underline{\textbf{-}} &- &-& \textbf{-} &\underline{\textbf{-}}&- &\underline{\textbf{-}} &\underline{\textbf{-}}\\

\bottomrule
\end{tabular}}
\caption{\textbf{Comparison to the state-of-the-art} on ShanghaiTech Part\_A, Part\_B, UCF\_QNRF, JHU-CROWD++ and TRANCOS.
%Our results set a new state-of-the-art on most datasets for most metrics.
We combine our three solutions with CSRNet+ and T2T-Vit to obtain counting results which are either competitive or better than the current state-of-the-art, highlighting their potential for density-based counting. \textbf{Bold} indicates the best density-based counting results, and \underline{underline} indicates the best overall counting approach.}
\label{tab:sota}
\end{table*}
%
%===============================
\subsection{Focus by simulating occlusion}
%===============================
In this experiment, we demonstrate the potential of our occlusion handling augmentation. To highlight effectiveness in highly occluded images, we divide the test images into two sets according to their occlusion level, as computed by Equation \ref{eq:occmap}. The test images are grouped into the \emph{low} occlusion set if their occlusion level is lower than $1.5$, the remaining images are grouped into the \emph{high} occlusion set. For ShanghaiTech Part\_A, we obtain 109 low and 73 high occlusion images and for UCF\_QNRF, we obtain 49 low and 285 high occlusion images. To highlight that the key here is occlusions, not just the augmentation, we have additionally investigated the effect of adding well-known occlusion augmentation approaches such as Cutout \citep{devries2017cutout} and CutMix \citep{yun2019cutmix}. The results are shown in Table \ref{tab:occlusion}. Compared to the base counting network CSRNet+, both Cutout and CutMix reduce the counting error, but cannot compete with our occlusion simulation (Part\_A: 61.2~\citep{devries2017cutout}, 60.6~\citep{yun2019cutmix}, and 59.1 for ours - UCF\_QNRF: 91.8~\citep{devries2017cutout}, 90.6~\citep{yun2019cutmix}, and 87.4 for ours). Especially, our approach works much better when occlusion levels are high (Part\_A: 95.0~\citep{devries2017cutout}, 94.3~\citep{yun2019cutmix}, and 91.2 for ours - UCF\_QNRF: 104.7~\citep{devries2017cutout}, 103.1~\citep{yun2019cutmix}, and 99.3 for ours). This experiment solidifies our point: occlusions weight heavily on the counting error, and there are not enough natural occlusions to learn from. Instead, by simulating occlusions, we can easily reduce the MAE effectively.

%===============================
\subsection{Comparative evaluation} \label{exp}
%===============================
For the final experiments, we first show the effect of combining the four ways of focus we propose for improving transformation from input images to density maps by repurposing point annotations. Then we compare to the state-of-the-art in counting. 

\textbf{Combining the three focuses.} Until now, we have established that every solution plays a significant role in counting on its own. In this study, we aim to assess whether these solutions are also complementary to each other. The results of this experiment are shown in Table \ref{tab:combine}, utilizing both CSRNet+ and T2T-Vit as backbones. Our approach incorporates foreground focus using cascading segmentation and foreground distillation (detailed in section \ref{sec:segmentation}), which effectively reduces MAE when compared to standard counting with only the base networks. Moreover, by combining either global density focus (section \ref{sec:global}) or focus by simulating occlusion (section \ref{sec:occlusion}), we were able to further decrease the MAE. When we combine all three solutions, we observe the lowest count error across datasets and base networks.
%
\begin{figure*}[h!]
\centering
\begin{subfigure}{0.244\textwidth}
\includegraphics[width=\textwidth]{figures/case/case_img.pdf}
\caption{\textbf{Input image}}
\label{fig:augmentation-a}    
\end{subfigure}
\begin{subfigure}{0.246\textwidth}
\includegraphics[width=\textwidth]{figures/case/case_seg.pdf}
\caption{\textbf{Cascade image}}
\label{fig:augmentation-b}    
\end{subfigure}
\begin{subfigure}{0.243\textwidth}
\includegraphics[width=\textwidth]{figures/case/case_density.pdf}
\caption{\textbf{Our density}}
\label{fig:augmentation-c}    
\end{subfigure}
\begin{subfigure}{0.243\textwidth}
\includegraphics[width=\textwidth]{figures/case/case_gt.pdf}
\caption{\textbf{Ground-truth}}
\label{fig:augmentation-d}    
\end{subfigure}
\caption{\textbf{Success and failure cases.} Illustrative examples of success and failure cases. When objects are individually visible, we can count them accurately (first three rows). Further improvements are required for extremely dense scenes where individual objects are hard to distinguish, or where objects blend with the context (last two rows). }
\label{fig:cases}    
\end{figure*}

\textbf{Comparison to the state-of-the-art.}
As the ultimate test, we draw a comparison to the state-of-the-art in counting on five datasets.
We report our results using both CSRNet+ and T2T-Vit as base networks, and both $ell_1$ and distribution matching (DM) \cite{wang2020distribution} as loss functions. Table \ref{tab:sota} shows the comparative evaluation over all datasets and metrics. The results show that despite using canonical counting backbones, which on their own can not compete with the state-of-the-art, we obtain the best density-based counting results on 8 of the 10 metrics. This highlights the potential of our simple solutions. We also compare to recent point-based counting alternatives and find that we maintain the best results for 6 of the 10 metrics. On ShanghaiTech Part\_A, we score below 50 in terms of MAE for the first time. We conclude that with our proposed solutions, we can make density-based optimization the most effective way to count again.
%
We show some success and failure results in Figure~\ref{fig:cases}. Even in challenging scenes with relatively sparse small objects or relatively dense large objects, our method is able to achieve an accurate count (first three rows). Our approach fails when dealing with extremely dense scenes where individual objects are hard to distinguish, or where objects blend with the context (last two rows). Such scenarios remain open counting challenges.

%\subsection{More analysis}
%\textbf{Complexity analysis.}
%The distilled density maps and occlusion simulations do not change inference time. Only the segmentation cascade adds complexity and increases the inference time, \eg, from 0.27s to 0.53s per image for the UCF\_QNRF dataset.
%\psmm{Do we have more analyses? Otherwise better to add this text to the implementation details.}
%The occlusion simulation relies on the size of objects. Currently, we use $2\sigma$ as an approximation to the size of an object. Since $\sigma$ is not estimated perfectly, a part of objects or the background is likely copied, which may affect the counting performance.
